Model-Based Reinforcement Learning for Atari

Model-free reinforcement learning (RL) can be used to learn effective policies for complex tasks, such as Atari games, even from image observations. However, this typically requires very large amounts of interaction -- substantially more, in fact, than a human would need to learn the same games. How can people learn so quickly? Part of the answer may be that people can learn how the game works and predict which actions will lead to desirable outcomes. In this paper, we explore how video prediction models can similarly enable agents to solve Atari games with fewer interactions than model-free methods. We describe Simulated Policy Learning (SimPLe), a complete model-based deep RL algorithm based on video prediction models and present a comparison of several model architectures, including a novel architecture that yields the best results in our setting. Our experiments evaluate SimPLe on a range of Atari games in low data regime of 100k interactions between the agent and the environment, which corresponds to two hours of real-time play. In most games SimPLe outperforms state-of-the-art model-free algorithms, in some games by over an order of magnitude.

==> SimPLe_ICRL_submission/analysis.tex <==
\section{Experiments}
\label{sec:experiments}
\label{sec:analysis}

\iffalse
\setlength{\tabcolsep}{3pt}
\begin{table}
\scriptsize
\caption{Mean scores obtained by our method (SimPLe) in comparison with Rainbow trained on 100K steps (400K frames) and PPO trained on 500K steps (2 millions frames). Details and extended numerical results are included in Appendix~\ref{numerical_results}.}
\begin{tabular}{lrrrrr}

Game &          SimPLe (ours)  &     rainbow\_100k &     ppo\_500k   &     human &          random \\

\midrule
Alien          &    405.2 &    290.6 &    269.0 &   7128.0 &   184.8 \\
Amidar         &     88.0 &     20.8 &     93.2 &   1720.0 &    11.8 \\
Assault        &    369.3 &    300.3 &    552.3 &    742.0 &   233.7 \\
Asterix        &   1089.5 &    285.7 &   1085.0 &   8503.0 &   248.8 \\
BankHeist      &      8.2 &     34.5 &    641.0 &    753.0 &    15.0 \\
BattleZone     &   5184.4 &   3363.5 &  14400.0 &  37188.0 &  2895.0 \\
Boxing         &      9.1 &      0.9 &      3.5 &     12.0 &     0.3 \\
Breakout       &     12.7 &      3.3 &     66.1 &     30.0 &     0.9 \\
ChopperCommand &   1246.9 &    776.6 &    860.0 &   7388.0 &   671.0 \\
CrazyClimber   &  39827.8 &  12558.3 &  33420.0 &  35829.0 &  7339.5 \\
DemonAttack    &    169.5 &    431.6 &    216.5 &   1971.0 &   140.0 \\
Freeway        &     20.3 &      0.1 &     14.0 &     30.0 &     0.0 \\
Frostbite      &    254.7 &    140.1 &    214.0 &      - &    74.0 \\
Gopher         &    771.0 &    748.3 &    560.0 &   2412.0 &   245.9 \\
Hero           &   1295.1 &   2676.3 &   1824.0 &  30826.0 &   224.6 \\
Jamesbond      &    125.3 &     61.7 &    255.0 &    303.0 &    29.2 \\
Kangaroo       &    323.1 &     38.7 &    340.0 &   3035.0 &    42.0 \\
Krull          &   4539.9 &   2978.8 &   3056.1 &   2666.0 &  1543.3 \\
KungFuMaster   &  17257.2 &   1019.4 &  17370.0 &  22736.0 &   616.5 \\
MsPacman       &    762.8 &    364.3 &    306.0 &   6952.0 &   235.2 \\
Pong           &      5.2 &    -19.5 &     -8.6 &     15.0 &   -20.4 \\
PrivateEye     &     58.3 &     42.1 &     20.0 &  69571.0 &    26.6 \\
Qbert          &    559.8 &    235.6 &    757.5 &  13455.0 &   166.1 \\
RoadRunner     &   5169.4 &    524.1 &   5750.0 &   7845.0 &     0.0 \\
Seaquest       &    370.9 &    206.3 &    692.0 &  42055.0 &    61.1 \\
UpNDown        &   2152.6 &   1346.3 &  12126.0 &  11693.0 &   488.4 \\
\bottomrule
\end{tabular}
\label{tab:shortNumericalResults}
\end{table}
\fi

We evaluate SimPLe on a suite of Atari games from Atari Learning Environment (ALE) benchmark.
In our experiments, the training loop is repeated for 15 iterations, with $6400$ interactions with the environment collected in each iteration.
We apply a standard pre-processing for Atari games: a frame skip equal to 4, that is every action
is repeated 4 times. The frames are down-scaled by a factor of $2$.

Because some data is collected before the first iteration of the loop,
altogether $6400 \cdot 16 = 102,400$ interactions with the Atari environment are used during training.
This is equivalent to $409,600$ frames from the Atari game (114 minutes at 60 FPS).
At every iteration, the latest policy trained under the learned model is used to collect data in the real environment $\env$.
% BO 2020/02/12.
The data is also directly used to train the policy with PPO.
Due to vast difference between number of training data from simulated environment and real environment (15M vs 100K) the impact of the latter on policy is negligible.
% as part of the Tensor2Tensor library with instructions on how to run our experiments.\footnote{\url{https://github.com/tensorflow/tensor2tensor/tree/master/tensor2tensor/rl}} 

We evaluate our method on $26$ games selected on the basis of being solvable with existing state-of-the-art model-free deep RL algorithms\footnote{Specifically, for the final evaluation we selected games which achieved non-random results using our method or the Rainbow algorithm using $100$K interactions.}, which in our comparisons are Rainbow~\cite{rainbow} and PPO~\cite{ppo}. For Rainbow, we used the implementation from the Dopamine package and spent considerable time tuning it for sample efficiency (see Appendix \ref{sec:baselines_optimizations}).

For visualization of all experiments see \url{https://goo.gl/itykP8}
and for a summary see Figure~\ref{fig:compare_dopamine_ppo}.
It can be seen that our method is more sample-efficient than a highly tuned Rainbow baseline on almost all games, requires less than half of the samples on more than half of the games and, on {\freeway}, is more than 10x more sample-efficient. Our method outperforms PPO by an even larger margin.
We also compare our method with fixed score baselines (for different baselines) rather than counting how many steps are required to match our score, see Figure~\ref{fig:compare_scores} for the results.
For the qualitative analysis of performance on different games see Appendix \ref{qualitative_analysis}.
The source code is available as part of the Tensor2Tensor library and it includes instructions on how to run the experiments\footnote{\url{https://github.com/tensorflow/tensor2tensor/tree/master/tensor2tensor/rl}}.

\begin{figure}
\centering
\includegraphics[width=0.45\columnwidth]{figures/v1_eval_longmodel_vs_rainbow-1.png}
\includegraphics[width=0.45\columnwidth]{figures/v1_eval_longmodel_vs_ppo-1.png}
\vspace{-0.2cm}
\caption{Comparison with Rainbow and PPO. Each bar illustrates the number of interactions with environment required by Rainbow (left) or PPO (right) to achieve the same score as our method (SimPLe). The red line indicates the $100$K interactions threshold which is used by the our method.} 
\label{fig:compare_dopamine_ppo}
\vspace{-0.5cm}
\end{figure}


\subsection{Sample Efficiency}
The primary evaluation in our experiments studies the sample efficiency of SimPLe, in comparison with state-of-the-art model-free deep RL methods in the literature. To that end, we compare with  Rainbow~\citep{rainbow,DBLP:journals/corr/abs-1812-06110}, which represents the state-of-the-art Q-learning method for Atari games, and PPO~\citep{ppo}, a model-free policy gradient algorithm (see Appendix \ref{sec:baselines_optimizations} for details of tuning of Rainbow and PPO). The results of the comparison are presented in Figure~\ref{fig:compare_dopamine_ppo}. For each game, we plot the number of time steps needed for either Rainbow or PPO to reach the same score that our method reaches after $100$K interaction steps. The red line indicates $100$K steps: any bar larger than this indicates a game where the model-free method required more steps. SimPLe outperforms the model-free algorithms in terms of learning speed on nearly all of the games, and in the case of a few games, does so by over an order of magnitude. For some games, it reaches the same performance that our PPO implementation reaches at $10$M steps. This indicates that model-based reinforcement learning provides an effective approach to learning Atari games, at a fraction of the sample complexity.

The results in these figures % and Table \ref{tab:shortNumericalResults}
are generated by averaging $5$ runs for each game.
% As shown in Table \ref{tab:shortNumericalResults},
The model-based agent is better than a random policy for all the games except \bankh. Interestingly, we observed that the best of the $5$ runs was often significantly better. For $6$ of the games, it exceeds the average human score (as reported in Table 3 of \cite{Pohlenetal2018}). This suggests that further stabilizing SimPLe should improve its performance, indicating an important direction for future work. In some cases during training  we observed high variance of the results during each step of the loop. There are a number of possible reasons, such as mutual interactions of the policy training and the supervised training or domain mismatch between the model and the real environment. We present detailed numerical results, including best scores and standard deviations, in Appendix \ref{numerical_results}.

\begin{figure}
\centering
\includegraphics[width=0.245\columnwidth]{figures/nfraction_of_rainbow_at_100K.png}
\includegraphics[width=0.245\columnwidth]{figures/nfraction_of_rainbow_at_200K.png}
\includegraphics[width=0.245\columnwidth]{figures/nfraction_of_ppo_at_100K.png}
\includegraphics[width=0.245\columnwidth]{figures/nfraction_of_ppo_at_200K.png}
\vspace{-0.2cm}
\caption{Fractions of Rainbow and PPO scores at different numbers of interactions calculated with the formula $(SimPLe\_score@100K - random\_score)/(baseline\_score - random\_score)$; if denominator is smaller than 0, both nominator and denominator are increased by 1. From left to right, the baselines are: Rainbow at 100K, Rainbow at 200K, PPO at 100K, PPO at 200K.
SimPLe outperforms Rainbow and PPO even when those are given twice as many interactions.}
\label{fig:compare_scores}
\vspace{-0.5cm}
\end{figure}

\subsection{Number of frames}

We focused our work on learning games with $100$K interaction steps with the environment. In this section we present additional results for settings with $20$K, $50$K, $200$K, $500$K and $1$M interactions; see Figure~\ref{fig:numberOfStepsMT}~(a).
Our results are poor with $20$K interactions. For $50$K they are already almost as good as with $100$K interactions. From there the results improve until $500$K samples -- it is also the point at which they are on par with model-free PPO. Detailed per game results can be found in Appendix~\ref{appdx:num_samples}.

This demonstrates that SimPLe excels in a low data regime, but its advantage disappears with a bigger amount of data.
Such a behavior, with fast growth at the beginning of training, but lower asymptotic performance is commonly observed when comparing model-based and model-free methods (\citet{benchmarkingmbrl}). As observed in Section \ref{subabl} assigning bigger computational budget helps in $100$K setting. We suspect that gains would be even bigger for the settings with more samples. 
% The limitation of the presented results is that even with the highest number of frames, the method was assigned the same computational budget as for $100$K interactions. As suggested by Section \ref{subabl}, we could expect further improvement to the performance with prolonging model training.

Finally, we verified if a model obtained with SimPLe using $100$K is a useful initialization for model-free PPO training. 
Based on the results depicted in Figure~\ref{fig:numberOfStepsMT}~(b) we can positively answer this conjecture. Lower asymptotic performance is probably due to worse exploration. A policy pre-trained with SimPLe was meant to obtain the best performance on $100$K, at which point its entropy is very low thus hindering further PPO training.

\newcommand{\mywidth}{3.5in}
\begin{figure}
\begin{tabular}{@{\hskip -3em}c@{\hskip -3.5em}c}
\subfloat[Model based (SimPLe)]{\includegraphics[width = \mywidth ]{figures/number_of_step_simple.pdf}} &
\subfloat[Model based + model free (SimPLe + PPO)]{\includegraphics[width = \mywidth]{figures/number_of_step_simple_ppo.pdf}} 
\end{tabular}
\caption{Behaviour with respect to the number of used samples. We report number of frames required by PPO to reach the score of our models. Results are averaged over all games.\label{fig:numberOfStepsMT}}
\end{figure}

\subsection{Environment stochasticity}

A crucial decision in the design of world models is the inclusion of stochasticity. Although Atari is known to be a deterministic environment, it is stochastic given only a limited horizon of past observed frames (in our case $4$ frames). The level of stochasticity is game dependent; however, it can be observed in many Atari games.
% BO 2020/02/12
%An example of such behavior can be observed in the game \texttt{Kung Fu Master} -- after eliminating current set of opponents the game screen always looks the same (i.e. contains only player's character and the background). Based on this observation alone (and not the game internal state) it is most likely impossible to predict which opponents will emerge from behind the screen edge. A fully deterministic model would be bound to fail -- it could either keep predicting empty frames, or predict the same set of opponents, or a blurred image which average all potential opponents. As can be seen in Figure~\ref{fig:kungfu} in the Appendix the stochastic model learns a reasonable behavior -- samples potential opponents and renders them sharply.
An example of such behavior can be observed in the game \texttt{Kung Fu Master} -- after eliminating the current set of opponents, the game screen always looks the same (it contains only player's character and the background). The game dispatches diverse sets of new opponents, which cannot be inferred from the visual observation alone (without access to the game's internal state) and thus cannot be predicted by a deterministic model. Similar issues have been reported in \cite{sv2p}, where the output of their baseline deterministic model was a blurred superposition of possible random object movements. As can be seen in Figure~\ref{fig:kungfu} in the Appendix, the stochastic model learns a reasonable behavior -- samples potential opponents and renders them sharply.

\begin{wrapfigure}[26]{r}{0.45\textwidth}\label{fig:sticky}
\vspace{-0.5cm}
\includegraphics[width=0.45\textwidth]{figures/sticky_2}
%\vspace{-0.2cm}
\caption{Impact of the environment stochasticity.
%Comparison of experiments with and without sticky actions using stochastic discrete world models.
The graphs are in the same format as Figure~\ref{fig:compare_dopamine_ppo}: each bar illustrates the number of interactions with environment required by Rainbow to achieve the same score as SimPLe (with stochastic discrete world model) using 100k steps in an environment with and without sticky actions.}
\label{fig:sticky}
\end{wrapfigure}

Given the stochasticity of the proposed model, SimPLe can be used with truly stochastic environments. To demonstrate this, we ran an experiment where the full pipeline (both the world model and the policy) was trained in the presence of sticky actions, as recommended in \cite[Section 5]{ale2}. Our world model learned to account for the stickiness of actions and in most cases the end results were very similar to the ones for the deterministic case even without any tuning, see Figure~\ref{fig:sticky}.

\subsection{Ablations}\label{subabl}
To evaluate the design of our method, we independently varied a number of the design decisions. Here we present an overview; see Appendix~\ref{sec:ablations} for detailed results.
\vspace{0.1cm}\\\textbf{Model architecture and hyperparameters.}
We evaluated a few choices for the world model and our proposed stochastic discrete model performs best by a significant margin.
The second most important parameter was the length of world model's training. We verified that a longer training would be beneficial,
%but we had to restrict it because of a high cost of running the whole training on all Atari games.
however we had to restrict it in all other ablation studies due to a high cost of training on all games.
% but due to our resources constraints other ablations because were made with the short model training setting.
As for the length of rollouts from simulated $env'$, we use $N=50$ by default. We experimentally shown that $N=25$ performs roughly on par, while $N=100$ is slightly worse, likely due to compounding model errors.
%We experimented with $N=25$ or $N=100$ and $100$ is a bit worse than either $25$ or $50$ (which are on par), likely due to compounding model errors, but this effect is much smaller than the effect of model architecture.
The \emph{discount factor} was set to $\gamma=0.99$ unless specified otherwise.  We see that $\gamma=0.95$ is slightly better than other values, and we hypothesize that it is due to better tolerance to model imperfections. But overall, all three values of $\gamma$ perform comparably.
\vspace{0.1cm}\\\textbf{Model-based iterations.}
The iterative process of training the model, training the policy, and collecting data is crucial for non-trivial tasks where random data collection is insufficient. In a game-by-game analysis, we quantified the number of games where the best results were obtained in later iterations of training. In some games, good policies could be learned very early. While this might have been due to the high variability of training, it does suggest the possibility of much faster training (i.e. in fewer step than 100k) with more directed exploration policies. In Figure \ref{fig:Cdf} in the Appendix we present the cumulative distribution plot for the (first) point during learning when the maximum score for the run was achieved in the main training loop of Algorithm~\ref{alg:basic_loop}.
\vspace{0.1cm}\\\textbf{Random starts.} Using short rollouts is crucial to mitigate the compounding errors in the model. To ensure exploration, SimPLe starts rollouts from randomly selected states taken from the real data buffer $\textsc{D}$. Figure \ref{fig:Cdf} compares the baseline with an experiment without random starts and rollouts of length $1000$ on {\seaquest} which shows much worse results without random starts.

% \subsection{Qualitative Analysis}
% In addition to ablating parameters, we studied of individual games to better understand how SimPLe works. We emphasize that we did not adjust the method nor hyperparameters individually for each game, but we provide specific qualitative analysis to better understand our models.\footnote{We strongly encourage the reader to watch accompanying videos \url{https://goo.gl/itykP8}} 

% In some games (\pong, \freeway, \breakout) our models were able to predict the future pixel-perfect. In some other cases our models differed from the original games in a way that was harmless for policy training. For example, in {\bowling}, and {\pong}, the ball sometimes splits into two. While nonphysical, seemingly these errors did not distort much the objective of the game.

% In {\kungfumaster}, our model's predictions deviate from the real game by spawning a different number of opponents. In {\crazyclimber}, we observed the bird appearing earlier in the game. We attribute these cases to the stochasticity in the model. Though not aligned with the true environment, the predicted behaviors are plausible and the resulting policy can still play the original game.

% Finally, on some of the games, our models simply failed to produce useful predictions. The most common failure was due to the presence of very small but highly relevant objects. For example, in {\atlantis} and {\battlezone} bullets are so small that they tend to disappear. In Appendix~\ref{qualitative_analysis} we provide more detailed analysis.


==> SimPLe_ICRL_submission/analysis_old.tex <==
\section{Analysis}

To be included in this section
\begin{enumerate}
    \item ablation: number of training loops
    \item (?) ablation: PPO training on real env
    \item model measures (next frame accuracy, long term value prediction) don't determine final RL performance - how well we can justify it?
    \item  shared weights WM/P models
    \item effects of limited horizon -- e.g. pong/pacman doesn't restart, montezuma dies when jumping in place;
    bank heist story why stochastic model is better - not true?
    \item using of random starts is essential (?)
\end{enumerate}

\todo[inline]{All text in this section is just a placeholder; for mode details see the doc}
\label{envs}
\label{sec:envs}
% \todo[inline]{Here we describe interesting environments; this was quite nicely done in Chiappa's work as well as in Oh's work and this is the place where we want to discuss BankHeist}
In this section we describe \pong, \breakout\ and \freeway\ environments. These environments were introduced in the Arcade Learning Environment (ALE) \cite{ale} (see also \cite{ale2} for a current overview of challenges and successes of various learning methods in ALE). 

\paragraph{Dimensions of input and output.} The screen as given by the ALE emulator consists of an RGB image of the size $160\times 210$ pixels\todo[inline]{Is it rally true?}.  The action space consists of up to 18 actions\todo[inline]{MB.1.16: this is game dependent}. The reward in all games is an integer number\todo[inline]{MB.1.16: which we truncate to -1 0 and 1}.

\paragraph{\pong.} In \pong\ the player is expected to move the green paddle. The red paddle is operated by the original game AI. If the ball crosses the left end of the screen, then the green player scores a point. If the ball crosses the right end of the screen, then the red player scores a point. The total reward for the game is the difference between points scored by the green player and the red player. A full episode lasts until one of the agents scores 21 points. An environment for \pong\ was trained in \cite{recurrent}. Authors reported occasional disappearance of the ball and blurriness of paddles. In order to simplify learning of the environment we considered a modified environment with a ball of the size $10\times 10$ pixels. The change concerns only the observation and not rules of the game. 

\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__3.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__9.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__31.jpg}%
}%
\caption{Four frames from the \pong\ environment. }
\label{fig:pong_original}
\end{figure}


\paragraph{\breakout.} In \breakout\ the player is expected to move the paddle located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model, see page 18 of \cite{recurrent}. As in the case of \pong\ in the modified environment we allowed for a ball of the size $10\times 10$ pixels.

% \begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__2.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__3.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__6.jpg}%
}%
\caption{Four frames from the original \breakout\ environment. }
\label{fig:breakout_original}
\end{figure}
% \end{comment}

\begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__1.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__2.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__4.jpg}%
}%
\caption{Four frames from the modified \breakout\ environment. }
\label{fig:breakout_mod}
\end{figure}
\end{comment}

\paragraph{\freeway.} In \freeway\ the player is expected to move the yellow chicken from the bottom of the screen to the top of the screen.  The chicken moves only vertically. A point is obtained in the game if the chicken reaches the top of the screen. There is no concept of life, but if the chicken is hit by a car, then it falls approximately 2 lanes down. The environment makes appearance in \cite{recurrent} and is considered as an easy environment to model \cite[page 18]{recurrent} frames. The problem though are the sparse rewards, since the only time a non-0 reward occurs is at the top of the screen.  

%\begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__4.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__6.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__8.jpg}%
}%
\caption{Four frames from the original \freeway\ environment. }
\label{fig:breakout_mode}
\end{figure}
% \end{comment}

\paragraph{\bankh.} \todo[inline]{Here Łukasz includes his take on \bankh}


\paragraph{Improvements to performance over iterations}

We trained the iterative algorithm for 3 epochs of
the world-model/ppo/generate-data loop. In Figure~\ref{fig:freeway_three_epochs} we present
how the results change on the example of \freeway. Note that in the first step the environment is not producing rewards
correctly. It only learns to produce them in the second step and the results get high in the third. See the caption of the Figure and
\href{https://sites.google.com/view/modelbasedrlatari/home}{webpage}\footnote{\url{https://sites.google.com/view/modelbasedrlatari/home}} for 
videos showing progress of the agent. %[TODO: show chicken from the video unsure near the top?]

\begin{figure}[H]
\centering
\includegraphics[width=0.9\columnwidth]{figures/freeway.png}
%\includegraphics[width=1.8in]{figures/c0.png}
%\includegraphics[width=1.8in]{figures/c1.png}
%\includegraphics[width=1.8in]{figures/c3.png}
\caption{Three different runs of PPO training on simulated environment $env'$ for three iterations of the whole loop on \freeway\ training.
  The first iteration is epochs 0-50, the next 50-100 and the final one 100-150. Note that while all 3 models only reach scores below 4 in
  the shortened PPO training, all of them actually get scores above 10 when playing in the real environment, and the two better runs get above 20.
  Two of the runs already reach positive scores in the first iteration, while one run (orange) only reaches them in the second iteration -- this
  happens because no reward was seen in the first randomly generated data. In the third iteration the policies of the two runs that saw rewards
  in the first iteration get very good (scores above 20), while the third one learns slower.}
\label{fig:freeway_three_epochs}
\end{figure}

\paragraph{The accuracy metric on selected games.}\todo[inline]{(Henryk) @Piotr, I am assuming that you will fix it or remove}

\paragraph{Metrics}
We propose a new \textit{correct rewards predictions per sequence} metric to evaluate simulated environments. 
Let $t = (s, acs)$ be a tuple consisting of a state $s$ and a sequences of actions $acs$. We say that $env'$ is successful on $t$ if started from $s$ it produces the same total reward as the $env$ while executing subsequently actions $acs$.
Given $D$, a set of tuples as above we define \textit{correct rewards predictions per sequence} ratio on $D$ to be the ratio of successful $t$'s in $D$.
Typically, we evaluate simulated environment on $D$ with sequences $acs$ of a prescribed length $n\in \mathbb{N}$ generated according to some stochastically perturbed policy $\pi$. Intuitively, having good ratio in such a test means that the model behaves reliably in the neighborhood of $\pi$ in the time horizon $n$. %\todo{Piotr have a look here} %Thus, hopefully, it can be used in a reinforcement learning algorithm. 
We argue that this metric can correctly measure resemblance  of the simulated and original dynamics.  We believe it is better than the standard $L_2$ accuracy used in \cite{video_prediction,recurrent}, which has tendency to omit small but important objects (e.g. the ball in \pong).
\todo[inline]{So far we have one case: Pong, and number are very old, see Figure \ref{fig:correctness}}

\begin{figure}[H]
\includegraphics[width=0.35\textwidth]{figures/pong_ratio}%

\caption{Results on \pong: metric of correctness of rewards predictions per sequence.}
\label{fig:correctness}
\end{figure}

\paragraph{Analysis of the PPO modification}
\todo[inline]{So far we have one case: Pong, and number are very old, see Figure \ref{fig:ppo_mod}}

\begin{figure}[H]
\includegraphics[width=0.35\textwidth]{figures/compare1000steps}
\caption{Results on \pong: a comparison of training in two settings: one assuming 0 reward at the end of simulated environment episode and improved version using value function estimation instead.}
\label{fig:ppo_mod}
\end{figure}

==> SimPLe_ICRL_submission/architectures.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.88\textwidth]{figures/model_basic_disc.pdf}
\caption{Architecture of the proposed stochastic model with discrete latent. The input to the model is four stacked frames (as well as the action selected by the agent) while the output is the next predicted frame and expected reward. Input pixels and action are embedded using fully connected layers, and there is per-pixel softmax ($256$ colors) in the output. This model has two main components. First, the bottom part of the network which consists of a skip-connected convolutional encoder and decoder. To condition the output on the actions of the agent, the output of each layer in the decoder is multiplied with the (learned) embedded action. Second part of the model is a convolutional inference network which approximates the posterior given the next frame, similarly to~\citet{sv2p}. At training time, the sampled latent values from the approximated posterior will be discretized into bits. To keep the model differentiable, the backpropagation bypasses the discretization following~\citet{auto_discrete}. A third LSTM based network is trained to approximate each bit given the previous ones. At inference time, the latent bits are predicted auto-regressively using this network. The deterministic model has the same architecture as this figure but without the inference network.} 
\label{fig:full_discrete}
\vspace{-0.2cm}
\end{figure*}


\section{World Models}
\vspace{5pt}
\label{sec:world_models}
\label{sec:architectures}
\label{sec:training}


In search for an effective world model we experimented with various architectures, both new and modified versions of existing ones. This search resulted in a novel stochastic video prediction model (visualized in Figure~\ref{fig:full_discrete}) which achieved superior results compared to other previously proposed models. In this section, we describe the details of this architecture and the rationale behind our design decisions.  In Section \ref{sec:analysis} we compare the performance of these models.

\textbf{Deterministic Model.}
Our basic architecture, presented as part of Figure~\ref{fig:full_discrete}, resembles the convolutional feedforward network from \citet{video_prediction}.  The input $X$ consists of four consecutive game frames and an action $a$. Stacked convolution layers process the visual input. The actions are one-hot-encoded and embedded in a vector which is multiplied channel-wise with the output of the convolutional layers. 
The network outputs the next frame of the game and the value of the reward.%

In our experiments, we varied details of the architecture above. In most cases, we use a stack of four convolutional layers with $64$ filters followed by three dense layers (the first two have $1024$ neurons). The dense layers are concatenated with $64$ dimensional vector with a learnable action embedding. Next, three deconvolutional layers of $64$ filters follow. An additional deconvolutional layer outputs an image of the original $105\times 80$ size. The number of filters is either $3$ or $3 \times 256$. In the first case, the output is a real-valued approximation of pixel's RGB value. In the second case, filters are followed by softmax producing a probability distribution on the color space. The reward is predicted by a softmax attached to the last fully connected layer. 
We used dropout equal to $0.2$ and layer normalization. 

%TODO_PM_21_05: possibly say just shortely as below and move the two proceeding paragraphs to the appendix.
% For successful model training we found it crucial to use scheduled sampling \cite{BengioVJS15} and clipping of the loss function. Details are provided in Appendix~\ref{fill me please}.

\textbf{Loss functions.}
The visual output of our networks is either one float per pixel/channel or the categorical 256-dimensional softmax. In both cases, we used the \textit{clipped loss} $\max(Loss, C)$ for a constant $C$. We found that clipping was crucial for improving the models (measured with the correct reward predictions per sequence metric and successful training using Algorithm~\ref{dpll}). We conjecture that clipping substantially decreases the magnitude of gradients stemming from fine-tuning of big areas of background consequently letting the optimization process concentrate on small but important areas (e.g. the ball in Pong). In our experiments, we set $C=10$ for $L_2$ loss on pixel values and to $C=0.03$ for softmax loss.
Note that this means that when the level of confidence about the correct pixel value exceeds $97\%$  (as $-\ln(0.97) \approx 0.03$) we get no gradients from that pixel any longer.

\textbf{Scheduled sampling.}
The model $env'$ consumes its own predictions from previous steps and due to compounding errors, the model may drift out of the area of its applicability. Following \cite{BengioVJS15,venkatraman}, we mitigate this problem by randomly replacing in training some frames of the input $X$ by the prediction from the previous step while linearly increasing the mixing probability to $100\%$ around the middle of the first iteration of the training loop.

\textbf{Stochastic Models.}
A stochastic model can be used to deal with limited horizon of past observed frames as well as sprites occlusion and flickering which results to higher quality predictions. Inspired by~\citet{sv2p}, we tried a variational autoencoder~\citep{kingma2013auto} to model the stochasticity of the environment. In this model, an additional network receives the input frames as well as the future target frame as input and approximates the distribution of the posterior. At each timestep, a latent value $z_t$ is sampled from this distribution and passed as input to the original predictive model. At test time, the latent values are sampled from an assumed prior 
$\mathcal{N}(\mathbf{0}, \mathbf{I})$. 
To match the assumed prior and the approximate, we use the Kullback–Leibler divergence term as an additional loss term~\citep{sv2p}.

We noticed two major issues with the above model. First, the weight of the KL divergence loss term is game dependent, which is not practical if one wants to deal with a broad portfolio of Atari games. Second, this weight is usually a very small number in the range of $[10^{-3}, 10^{-5}]$ which means that the approximated posterior can diverge significantly from the assumed prior. This can result in previously unseen latent values at inference time that lead to poor predictions. We address these issues by utilizing a discrete latent variable similar to~\citet{auto_discrete}. 

As visualized in Figure~\ref{fig:full_discrete}, the proposed stochastic model with discrete latent variables discretizes the latent values into bits (zeros and ones) while training an auxiliary LSTM-based~\cite{hochreiter1997long} recurrent network to predict these bits autoregressively. At inference time, the latent bits will be generated by this auxiliary network in contrast to sampling from a prior. To make the predictive model more robust to unseen latent bits, we add uniform noise to approximated latent values before discretization and apply dropout~\citep{srivastava2014dropout} on bits after discretization. More details about the architecture is in Appendix \ref{sec:architecture-details}.




==> SimPLe_ICRL_submission/architectures_old.tex <==
\section{World models}
\label{sec:architectures}
\label{sec:training}

%%SL.12.27: Perhaps organizationally it would be better to first have a top-level Overview section to describe the parts of the method, and then a single top-level section with the name of the method, with subsections about the individual parts of the method? If the goal of this section is to discuss predictive model architectures, perhaps that would also make for a better section title: Predictive Model Architectures or something? The title of the first paragraph "Architecture of a Neural Simulator" could also work well (note however that in the deep learning community, "neural simulator" sometimes takes on a very specific meaning as an object-decomposed model that emulates the high-level design of a physics simulator)

% Dumitru. here is how I would structure this: 1-2 sentences about what we are looking for in a world model (stochasticity, scalability, stability). Say that to this end we came up with a new architecture that is straightforward but that is novel for video prediction. Also say that we compare with SV2P, and describe it. Then go into the details of the filter sizes and training losses: first the stuff that is common to both, then the specifics for each model. Alternative proposal is to describe the details of the world model training that are common first, and then describe the models themselves.}

%%SL.12.27: It could be a good idea at the beginning of this paragraph to explain the problems that the architecture design is trying to address so as to motivate the design decisions.
\paragraph{Architecture of a neural simulator of an environment. } Our basic architecture, presented in Figure~\ref{fig:kanapa}, resembles the convolutional feedforward network from \cite{video_prediction}.  The input $X$ consists of a few consecutive game frames and an action $a$. The visual input is processed by stacked convolution layers. The actions are one-hot-encoded and embedded in a vector which is multiplied channel-wise with the output of the conv layers. It is then processed by fully connected layers and deconvolved. The network outputs the next frame of the game and the value of reward.% Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

	In most of our experiments we choose the input to be four frames as with our choice of environments they fully identify the state of the game. The network is the workhorse of our simulated environment $env'$. The environment contains a memory $M$ of four frames, which is initialized with frames retrieved for the original environment. Given an action $a$ the tuple $(M,a)$ is processed by the network outputting a new frame and a reward $r$. The oldest frame of $M$ is discarded and the new one is included. 

%\todo{pm: The next section is too much of storytelling}
%\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games.
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design the same is true about the ouput $X'$.
%\todo{Important: no pooling}

In our experiments we varied details of the architecture above. In most cases we use a stack of four conv layers with $64$ filters followed by three dense layers (the first two have $1024$ neurons). The dense layers are concatenated with $64$ dimensional vector with a learnable action embedding. Next, three deconv layers of $64$ filters follow. An additional, final, deconv layer outputs an image of the original $210\times 160$ size. The number of filters is either $3$ or $2\times 256$. In the first case the output is a real-valued approximation of pixel's RGB value. In the second case filters are followed by softmax producing probability distribution on the color space. The reward is predicted by a softmax attached to the last fully connected layer. 
We used dropout equal to $0.2$ and the layer normalization. 

We have also experimented with Stochastic Variation Video Prediction (SV2P)~\cite{sv2p}, a recent technique that incorporates a latent variable model with a generative recurrent network. The latter is a convolutional LSTM from \cite{cdna} that internally predicts transformations of the context images conditioned on latent values, actions and the previous frames. The model is trained with the reparametrization trick and allows for efficient inference at test time. When successfully trained, it make it possible to sample diverse and plausible action-conditioned futures. For the Atari experiments, we followed the same protocol of training as with the basic convolutional model described above. Note that generally speaking the multiplier for the KL-loss $\beta$ has to be tuned on a per-game basis: we tried 3 such values per game (TODO: confirm with mbz how many we actually tried).\todo[inline]{The reference to KL-loss may require some elaboration or abstraction.}

% MB.1.17 commenting this out
% \begin{figure}[H]
% \centering
% \includegraphics[width=3.5in]{figures/sv2p}
% \caption{The Stochastic Variational Video Prediction model (SV2P) by \cite{sv2p}}
% \label{fig:sv2p}
% \end{figure} 

\paragraph{Loss functions}
The visual output of our networks are either one float per pixel/channel or the categorical 256-dimensional softmax. 
In the case of the real output we used the \textit{clipped $L_2$ loss}, viz. $\max(x^2 - C, 0), C>0$. We found that clipping was crucial for improving prediction power of the models (both measured with the correct rewards predictions per sequence metric and successful trainings using Algorithm \ref{dpll}). We conjecture that the clipping substantially decreases the magnitude of gradients stemming from fine-tuning of big areas of background consequently letting the optimization process to concentrate on small but important areas (e.g. the ball in Pong). Setting $C$ corresponding to $10$ pixels worked particularly well in our experiments. 
We used similar trick for the softmax outputs, namely we clipped the cross-entropy loss once the model achieved high level of confidence about a pixel value (we used $98\%$ in our experiments). As in the first case, clipping was crucial for obtaining well performing models. 

\paragraph{Scheduled sampling}
By design, the clipped loss does not produce accurate pictures. The simulator $env'$ consumes its own predictions from previous steps thus, due to compounding errors, the model may drift out of the area of its applicability. We mitigate this problem by randomly replacing in training some frames of the input $X$ by one step predictions. Typically, we increase the mixing probability during training arriving to $50\%$. 

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_det.pdf}
\caption{Architecture of deterministic model which consists of a skip-connected convolutional encoder and decoder. The input to the model is four stacked frames as well as the selected action while the output is the next predicted frame and expected reward. Input pixels and action are embedded using fully connected layers and there is per-pixel softmax ($256$ colors) in the output.}
\label{fig:model_det}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_stoch.pdf}
\caption{Architecture of stochastic model. The generative network is the same as Figure~\ref{fig:model_det} with an additional convolutional inference network to approximates the posterior given the next frame. The latent values will be sampled from approximated posterior and an assumed prior of $\mathcal{N}(\mathbf{0}, \mathbf{I})$ at training and inference time respectively.}
\label{fig:model_stoch}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_disc.pdf}
\caption{Architecture of stochastic model with discrete latent. The overall architecture of this models is similar to Figure~\ref{fig:model_stoch} with two main differences. First, at training time, the sampled latent values from the approximated posterior will be discretized into bits. The backpropagation bypasses the discretization similar to~\citet{van2017neural}. A third LSTM based network is trained to approximate each bit given the previous ones. At inference network, the latent bits are predicted auto-regressively using this network.} 
\label{fig:full_discrete}
\end{figure*}



% \section{Design and training of simulators}
% \label{sec:architectures}

% \paragraph{Architecture of a neural simulator of an environment. } Our basic architecture, see Figure \ref{fig:kanapa}, resembles the convolutional {\em feedforward} architecture from \cite{video_prediction}.  The input $X$ consists of $4$ game frames and the action $a$. The visual input is processed by stacked convolution layers. The actions are one-hot-encoded and then embedded in a vector which is concatenated with the the output of the conv layers. It is then processed by some fully connected layers and deconvolved. The output of the network is the next gameframe and the value of reward. Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

% %\todo{pm: The next section is too much of storytelling}
% %\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games. 
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design the same is true about the ouput $X'$. 
% %\todo{Important: no pooling}

% In our experiments we varied a number of layers, but the most standard architecture of the encoder consists of $4$ convolutional layers with 128 filters, followed by 3 dense layers. The third of the layers marked as $e$ in Figure \ref{fig:kanapa} is stacked with the embedding of actions marked as $a$ in Figure \ref{fig:kanapa}. The stacked layer is followed by $4$ deconvolutions.     

% \paragraph{Metrics}
% In our work we mostly abandonded $L_2$ metric as a measure of accurracy. We argue that in many cases it is not well suited to asses the models as it underweights meaning small (but potentially crucial) objects. Instead we introduce \textit{correct rewards per sequence} parametrized by the sequence length $n$. By definition the metric is the ratio of action sequences in the training/eval set for with $env'$ predicts total reward consistent with the one of $env$.

% \paragraph{Loss functions}
% Our experiments followed two lines. The first output was a single real value for each pixel and channel, in the second we used categorical output of 256-dimensional softmax. 

% For both losses we introduced a clipping factor: the final loss was $\max(loss - C, 0)$ for a constant $C>0$. We found that clipping was crucial for improving prediction power both over the standard $L_2$ loss and over the standard cross-entropy loss. We conjecture fine-tuneing of big areas of background the clipping substantially decreases the magnitued of gradients stemming from fine-tuneing of big areas of background consequnetly letting the optimisation process to concentrate on small but important areas, like the ball in Pong. We used $C = 0.01$ for cross-entropy loss (so the model did not get any benefit from being more than 99\% confident about any pixel value) and $C = 10$ for $L_2$ loss so
% that being within $3$ RGB values was considered sufficient.

% \paragraph{Mixing.} \todo{Add mixing}

% \paragraph{Resets.} \todo{Add resets}



%\cite{video_prediction,recurrent}. 
%Important points: the encoder-decoder architecture, prediction-dependent transition, observation-dependent transition, long-short term accuracy. 

%\paragraph{Training of a simulator of an environment}
%Some decisions.
%\todo[inline]{which models we want to discuss? Loss functions, layer details, mixing, metrics such as percent of successful trajectory-reward predictions, {\bf negative mining} (Henryk) Yes, we want to discuss, details of training to be described by Piotr}

%\input{figures/kanapa_network.tex}
% source: https://raw.githubusercontent.com/PetarV-/TikZ/master/Convolutional%20autoencoder/convolutional_autoencoder.tex
% overleaf copy (can be modified): https://www.overleaf.com/16266360vmyxnwdwdnpn

%Do we want a figure like\todo{The figure is missing actions and rewards, but this can be fixed}
% \begin{figure}[H]
% \centering
% \includegraphics[width=5.5in]{figures/new_arch.png}
% \caption{A simplified view of our encoder-decoder architecture.}
% \label{fig:kanapa}
% \end{figure}



==> SimPLe_ICRL_submission/big_unfinished_table.tex <==
% \paragraph{Big table}
% \setlength{\belowcaptionskip}{-17pt}
%\begin{wraptable}{r}{0.55\textwidth}
\begin{table}[H]
%\vspace{-17pt}
\begin{center}
{\scriptsize{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
Game          & random & ours@200K & ours@200(*) & ours@1M  & PPO@200K & PPO@1M & PPO@10M &  Dop \\
\hline
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
\hline
\end{tabular}
}}}
\end{center}
\label{tab:main}
\caption{Our model-based results for 42 games trained using various algorithms: 100K ours at 200K and 1M, ours@200(*)  - an impure version of our algorithm which is allowed to train on a real environment, PPO and Dopamina.}  
\end{table}

==> SimPLe_ICRL_submission/conclusion.tex <==
\section{Conclusions and Future Work}

We presented SimPLe, a model-based reinforcement learning approach that operates directly on raw pixel observations and learns effective policies to play games in the Atari Learning Environment. Our experiments demonstrate that SimPLe learns to play many of the games with just $100$K interactions with the environment, corresponding to 2 hours of play time. In many cases, the number of samples required for prior methods to learn to reach the same reward value is several times larger.

Our predictive model has stochastic latent variables so it can be applied in highly stochastic environments. Studying such environments is an exciting direction for future work, as is the study of other ways in which the predictive neural network model could be used. Our approach uses the model as a learned simulator and directly applies model-free policy learning to acquire the policy. However, we could use the model for planning. Also, since our model is differentiable, the additional information contained in its gradients could be incorporated into the reinforcement learning process. Finally, the representation learned by the predictive model is likely be more meaningful by itself than the raw pixel observations from the environment. Incorporating this representation into the policy could further accelerate and improve the reinforcement learning process.

While SimPLe is able to learn more quickly than model-free methods, it does have limitations. First, the final scores are on the whole lower than the best state-of-the-art model-free methods. This can be improved with better dynamics models and, while generally common with model-based RL algorithms, suggests an important direction for future work. Another, less obvious limitation is that the performance of our method generally varied substantially between different runs on the same game. The complex interactions between the model, policy, and data collection were likely responsible for this. In future work, models that capture uncertainty via Bayesian parameter posteriors or ensembles \citep{trpo_ensemble, Chua18} may improve robustness.
Finally, the computational and time requirement of training inside world model are substantial (see Appendix \ref{sec:architecture-details}), which makes developing lighter models an important research direction.

In this paper our focus was to demonstrate the capability and generality of SimPLe only across a suite of Atari games, however, we believe similar methods can be applied to other environments and tasks which is one of our main directions for future work. As a long-term challenge, we believe that model-based reinforcement learning based on stochastic predictive models represents a promising and highly efficient alternative to model-free RL. Applications of such approaches to both high-fidelity simulated environments and real-world data represent an exciting direction for future work that can enable highly efficient learning of behaviors from raw sensory inputs in domains such as robotics and autonomous driving.

\subsection*{Acknowledgments} We thank Marc Bellemare and Pablo Castro for their help with Rainbow and Dopamine. The work of Konrad Czechowski, Piotr Kozakowski and Piotr Miłoś was supported by the Polish National Science Center grants UMO-2017/26/E/ST6/00622. The work of Henryk Michalewski was supported by the Polish National Science Center grant UMO-2018/29/B/ST6/02959. This research was supported by the PL-Grid Infrastructure. In particular, Konrad Czechowski, Piotr Kozakowski, Henryk Michalewski, Piotr Miłoś and Błażej Osiński extensively used the Prometheus supercomputer, located in the Academic Computer Center
Cyfronet in the AGH University of Science and Technology in Kraków, Poland.
Some of the experiments were managed using \url{https://neptune.ai}. We would like to thank the Neptune team for providing us access to the team version and technical support.

==> SimPLe_ICRL_submission/conclusion_old.tex <==
\section{Conclusions and future work}

%%SL.1.22: Here is a suggested rephrasing of the paragraphs below (similar content, just organized a bit differently):
% We presented a model-based reinforcement learning approach that can operate directly on raw pixel observations, and can learn effective policies to play games in the Atari Learning Environment. Our experiments demonstrate that our approach can learn to play many of the games with just $100$K transitions, corresponding to ??? hours of play time. In many cases, the number of samples required for prior methods to learn to reach the same reward value is several times larger.
%
% While the predictive model in our experiments has stochastic latent variables, the Atari games that we evaluate on are largely deterministic. Studying stochastic domains is an exciting direction for future, and we expect that effective probabilistic modeling of dynamics would be effective in such settings also. Another interesting direction for future work is to study other ways in which the predictive neural network model could be used. Our approach utilizes the model as a learned simulator, and then directly uses model-free policy search methods to acquire the behavior policy. However, since neural network models are differentiable, the additional information contained in the dynamics gradients could itself be incorporated into the reinforcement learning process. Finally, the representation learned by the predictive model is likely to itself be more meaningful than the raw pixel observations from the environment, and incorporating this representation into the policy could further accelerate and improve the reinforcement learning process.
%
% As a long-term challenge, we believe that model-based reinforcement learning based on stochastic predictive models represents a promising and highly efficient alternative to model-free RL, and applications of such approaches to both high-fidelity simulated environments and real-world data represent an exciting direction for future work that can enable highly efficient learning of behaviors from raw sensory inputs, in domains such as robotics and autonomous driving.

%%SL.1.22: Some general rationale: let's try to keep prior work to the prior work section, it often comes across as pretty unsatisfying to have a discussion section that says something like "prior word did this, maybe we can do it too in future work" (if it was done in prior work, then it's not future work). It's also important to leave the reader with a very positive impression of the work, so while discussing some limitations is really important, it's also a good idea to use these to frame exciting future work that goes beyond the current method.

We presented a number of ideas that, taken together, allow to train Atari games end-to-end in a model-based way and get improvements in data efficiency.
While in this work we focus on deterministic environments, it would be interesting to study stochastic environments, possibly exploiting methods from \cite{world_models}. This would open possibly of using model-based reinforcement learning techniques in real-world unstructured scenarios, for example competing in a video game against human players. 

In some of our experiments we output probability distributions over pixel values. We conjecture that their entropy/variance can serve a measure how model is confident about its own predictions. We mention \cite{trpo_ensemble} which introduced model ensembles with a similar purpose. Measuring confidence is a challenging task with multiple possible applications. On the one hand, it might be used to determine trust regions for policy optimization, resulting in a more stable execution of Algorithm~\ref{alg:basic_loop}. On the other hand, creating an incentive to enter low confidence regions might be a useful exploration strategy. 

Finally, there are many benefits of having a neural net model of a game. Its hidden state is smaller and possibly more semantically meaningful than visual input and could be used as an input for policy. As called for in \cite{modelplanning}, one could use it for model-based planning and propagate gradients though the model. Finally, there are many technical benefits as the neural network model runs on the same accelerator that trains the policy and can be ran in batch mode, greatly simplifying the architecture of the RL setup and speeding up computations for more complex environments.

As a long-term challenge, we would like to deal with visually rich simulated robotics environments such like Carla \cite{carla}. Compressing states as shown in \cite{world_models} is particularly appealing as such approach could be used in mixed scenario where the compression is learn using simulated data and later used for rapid reinforcement learning on real-world data. 

==> SimPLe_ICRL_submission/environments.tex <==
\section{Atari environments}
\label{envs}
\label{sec:envs}
% \todo[inline]{Here we describe interesting environments; this was quite nicely done in Chiappa's work as well as in Oh's work and this is the place where we want to discuss BankHeist}
In this section we describe \pong, \breakout\ and \freeway\ environments. These environments were introduced in the Arcade Learning Environment (ALE) \cite{ale} (see also \cite{ale2} for a current overview of challenges and successes of various learning methods in ALE). 

\paragraph{Dimensions of input and output.} The screen as given by the ALE emulator consists of an RGB image of the size $160\times 210$ pixels\todo[inline]{Is it rally true?}.  The action space consists of up to 18 actions. The reward in all games is an integer number.

\paragraph{\pong.} In \pong\ the player is expected to move the green paddle. The red paddle is operated by the original game AI. If the ball crosses the left end of the screen, then the green player scores a point. If the ball crosses the right end of the screen, then the red player scores a point. The total reward for the game is the difference between points scored by the green player and the red player. A full episode lasts until one of the agents scores 21 points. An environment for \pong\ was trained in \cite{recurrent}. Authors reported occasional disappearance of the ball and blurriness of paddles. In order to simplify learning of the environment we considered a modified environment with a ball of the size $10\times 10$ pixels. The change concerns only the observation and not rules of the game. 

\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__3.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__9.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__31.jpg}%
}%
\caption{Four frames from the \pong\ environment. }
\label{fig:pong_original}
\end{figure}


\paragraph{\breakout.} In \breakout\ the player is expected to move the paddle located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model \cite[page 18]{recurrent}. As in the case of \pong\ in the modified environment we allowed for a ball of the size $10\times 10$ pixels.

%\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__2.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__3.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__6.jpg}%
}%
\caption{Four frames from the original \breakout\ environment. }
\label{fig:breakout_original}
\end{figure}
%\end{comment}

\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__1.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__2.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__4.jpg}%
}%
\caption{Four frames from the modified \breakout\ environment. }
\label{fig:breakout_mod}
\end{figure}
\end{comment}

\paragraph{\freeway.} In \freeway\ the player is expected to move the yellow chicken from the bottom of the screen to the top of the screen.  The chicken moves only vertically. A point is obtained in the game if the chicken reaches the top of the screen. There is no concept of life, but if the chicken is hit by a car, then it falls approximately 2 lanes down. The environment makes appearance in \cite{recurrent} and is considered as an easy environment to model \cite[page 18]{recurrent} frames. The problem though are the sparse rewards, since the only time a non-0 reward occurs is at the top of the screen.   % located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model \cite[page 18]{recurrent}.  

%\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__4.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__6.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__8.jpg}%
}%
\caption{Four frames from the original \freeway\ environment. }
\label{fig:breakout_mode}
\end{figure}
% \end{comment}

\paragraph{\bankh.} \todo[inline]{Here Łukasz includes his take on \bankh}


==> SimPLe_ICRL_submission/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate SimPLe on a suite of Atari games from Atari Learning Environment (ALE) benchmark.
In our experiments, the training loop is repeated for 15 iterations, with $6400$ interactions with the environment collected in each iteration.
We apply a standard pre-processing for Atari games: a frame skip equal to 4, that is every action
is repeated 4 times and frames are down-scaled by a factor of 2.

Because some data is collected before the first iteration of the loop,
altogether $6400 \cdot 16 = 102,400$ interactions with the Atari environment are used during training.
This is equivalent to $409,600$ frames from the Atari game (114 minutes in NTCS, 60 FPS).
All our code is available. \textbf{TODO: more?}
% as part of the Tensor2Tensor library with instructions on how to run our experiments.\footnote{\url{https://github.com/tensorflow/tensor2tensor/tree/master/tensor2tensor/rl}} 

At every iteration, the latest policy trained under the learned model is used to collect data in the real environment $\env$.
Due to vast difference between number of training data from simulated environment and real environment (15M vs 100K) the impact of real data on policy is negligible.

 We evaluate our method on $26$ games selected on the basis of being solvable with existing state-of-the-art model-free deep RL algorithms\footnote{Specifically, for the final evaluation we selected games which achieved non-random results using our method or the Rainbow algorithm using $100$K interactions.}, which in our comparisons are Rainbow~\citep{rainbow} and PPO~\citep{ppo}.
 For Rainbow, we used the implementation from the Dopamine package and spent considerable time tuning it for sample efficiency.

For visualization of all experiments see \url{https://goo.gl/itykP8}
and for a summary see Figures \ref{fig:compare_dopamine} and  \ref{fig:compare_ppo}.
It can be seen that our method is more sample-efficient than a highly tuned Rainbow baseline on almost all games, requires less than half of the samples on more than half of the games and, on \freeway\, is more than 10x more sample-efficient. Our method outperforms PPO by an even larger margin.


==> SimPLe_ICRL_submission/figures/kanapa_network.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.1,every node/.style={scale=0.1}]]

	\node (1) [draw, dashed, minimum height=15em, minimum width=62em, xshift=24em, fill=olivegreen, fill opacity=0.2, very thick, rectangle, rounded corners] {};
		\node (la1) [below=0em of 1] {{\emph{encoder}}};
	\node (2) [draw, dashed, minimum height=14em, fill = red, fill opacity=0.2,minimum width=35em, xshift=63.5em, very thick, rectangle, rounded corners] {};
		\node (la1) [below=0em of 2] {{\emph{decoder}}};

	\node[] (i2) {};
	\pic[fill=green!50] (I2) {cube={1.8/1.8/0.4/1}};
	
	\togglefalse{redraw}
	\togglefalse{redraw2}
	
  	\node[right=16em of i2] (y) {};
  	
  	\pic[right=16em of i2, fill=echoreg!50] (Y) {cube={1.8/1.8/1/1}};
  	
  	\node[right=12em of y] (y1) {};
  	\pic[right=12em of y, fill=red!50] (Y1) {cube={0.9/0.9/1/1}};
  	
  	\node[right=12em of y1] (y2) {};
  	\pic[right=12em of y1, fill=echoreg!50] (Y2) {cube={0.9/0.9/2/1}};
  	\node[right=10em of y2] (y3) {};
  	\pic[right=10em of y2, fill=red!50] (Y3) {cube={0.45/0.45/2/1}};
  	
  	\node[right=9em of y3] (z1) {};
  	\pic[right=9em of y3, fill=mymauve!50] (Z1) {cube={0.9/0.9/1/1}};
  	
  	\node[right=12em of z1] (z2) {};
  	\pic[right=12em of z1, fill=mymauve!50] (Z2) {cube={1.8/1.8/0.4/1}};
  	
  	\draw [-stealth, ultra thick] (I2-B) -- node[above] {Conv.} node[below] {ReLU} (Y-A);
  	
  	\draw [-stealth, ultra thick] (Y-B) -- node[above] {Pool} (Y1-A);
  	
  	\draw [-stealth, ultra thick] (Y1-B) -- node[above=0.3em, inner sep=0.1em] {Conv.} node[below] {ReLU} (Y2-A);
  
  	\draw [-stealth, ultra thick] (Y2-B) -- node[above] {Pool} (Y3-A);
  	
  	
  	\draw [-stealth, ultra thick] (Y3-B) -- node[above] {Deconv.} node[below] {ReLU} (Z1-A);
  	
  	\draw [-stealth, ultra thick] (Z1-B) -- node[above] {Deconv.} node[below] {logistic} (Z2-A);
  	
  	
  	\color{black}
  	
  	\toggletrue{redraw}
  	\toggletrue{redraw2}
  	
  	\node[right=16em of i2] (y) {};
  	\pic[right=16em of i2, fill=echoreg!50] (Y) {cube={1.8/1.8/1/1}};
  	
  	\pic[right=12em of y, fill=red!50] (Y1) {cube={0.9/0.9/1/1}};
  	
  	\pic[right=12em of y1, fill=echoreg!50] (Y2) {cube={0.9/0.9/2/1}};
  	
  	\pic[right=9em of y3, fill=mymauve!50] (Z1) {cube={0.9/0.9/1/1}};
  	
  	\togglefalse{redraw2}
  	
  	\pic[right=10em of y2, fill=red!50] (Y3) {cube={0.45/0.45/2/1}};
  	
  	\toggletrue{redraw2}
  	
	\node[] (i2) {\LARGE ${\bf X}$};
  	\node[right=9.25em of y2] (y3) {\LARGE ${\bf z}$};
  	\node[right=11em of z1] (z2) {\LARGE ${\bf X}'$};

\end{tikzpicture}
\label{fig:kanapa_net}
\end{figure}

==> SimPLe_ICRL_submission/figures/the_loop.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}[node distance = 0.9cm, thick, scale=1., 
every node/.style={scale=1.}, nodes = {align = center},>=latex]
  \node[Minimum Width = loop, shape = ellipse, fill = red] (imp-sol)
    {\texttt{Gather observations and rewards using $\pi$ in $\env$}\\ 
    \texttt{and use them to improve model $\env'$}};
  \node[Minimum Width = loop, fill = yellow, below = of imp-sol] (rec-box)
    {\texttt{train $\pi$ in $\env'$}\\ \texttt{using a model-free algorithm}};
  \node[shift = (left:.7*x_node_dist)] at
    ($(imp-sol.west|-imp-sol.south)!.5!(rec-box.north west)$) (for-1) {};
  \node[above = of for-1] (for-3) {};
    % {$\texttt{action}$};
  \node[shift = (right:.7*x_node_dist),minimum size = 0pt] at
    ($(imp-sol.east|-imp-sol.south)!.5!(rec-box.north east)$) (for-2) {};
  \node[above = of for-2] (for-4) {};
    % {$\texttt{state}$};
  \begin{scope}[on background layer]
    \node[fit = (for-1)(for-2)(imp-sol)(rec-box), basic box = blue,
      header = Vanilla model-based RL loop] (dmft-l) {};
  \end{scope}
  % \draw[->] (rec-box) |- ++(1,-1) |- (imp-sol);
  % \path[very thick, blue, hv] (rec-box) edge[->] (for-1) edge[<-] (imp-sol);
  \path[very thick, blue, hv] (rec-box) edge[-] (for-3) edge[<-] (for-4)
                              (imp-sol) edge[-] (for-4) edge[<-] (for-3);

%  \node[left = of dmft-l, basic box = green, header = Corpus]
%    (dmft-p) {};
%  \path[fat blue line, ->, dashed, vh] (dmft-p) edge
%    ({$(dmft-p.east)$}-|dmft-l.west);
\end{tikzpicture}
\caption{The learning model-based learning loop; $\env$ is the original game and $\env'$ is a simulator of $\env$. }
\label{figure_basic_loop}
\end{figure}

==> SimPLe_ICRL_submission/figures_mod/architectures.tex <==
\section{World Models}
\label{sec:world_models}
\label{sec:architectures}
\label{sec:training}

%\begin{comment}
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{figures/model_basic_disc.pdf}
%\includegraphics[width=1.\textwidth]{figures/cycle.pdf}
\caption{Architecture of the proposed stochastic model with discrete latent. The input to the model is four stacked frames (as well as the action selected by the agent) while the output is the next predicted frame and expected reward. Input pixels and action are embedded using fully connected layers, and there is per-pixel softmax ($256$ colors) in the output. This model has two main components. First, the bottom part of the network which consists of a skip-connected convolutional encoder and decoder. To condition the output on the actions of the agent, the output of each layer in the decoder is multiplied with the (learned) embedded action. Second part of the model is a convolutional inference network which approximates the posterior given the next frame similar to~\citet{sv2p}. At training time, the sampled latent values from the approximated posterior will be discretized into bits. To keep the model differentiable, the backpropagation bypasses the discretization following~\citet{auto_discrete}. A third LSTM based network is trained to approximate each bit given the previous ones. At inference time, the latent bits are predicted auto-regressively using this network. The deterministic model has the same architecture as this figure but without the inference network.} 
\label{fig:full_discrete}
\end{figure*}
% \end{comment}


% In principle any model that approximates the following transition function can be used as a world model:
%$$
% $(s_{t+1}, r_{t+1}) = T(s_{0:t}, a_{0:t})$
%$$
% where $s_t, a_t,$ and $r_t$ are the state, action and reward at time-step $t$. Hence, any world model has two major components: next frame predictor and reward predictor. 

%In practice, scalability and stability of a model are crucial which limits the practicality of current video prediction models. We found out that merging the reward predictor and frame predictor helps with both performance and convergence speed. More precisely, merging the reward model can help the next frame predictor to get \textit{more important} pixels right whereas in the absence of such signal the video model receives an equal penalty for each pixel.

A crucial decision in the design of world models   % introduced in Section \ref{sec:mbrl}
% Another crucial design element for designing an effective world model 
is the inclusion of stochasticity. Although Atari is known to be a deterministic environment, it is stochastic given only a limited horizon of past observed frames (in our case $4$ frames). The level of stochasticity is game dependent; however, it can be observed in many Atari games. An example of such behavior is the \textit{pause} after a player scores in \texttt{Pong}. These pauses are longer than 4 frames, so a model looking at only the past 4 frames does not know when a new round of the game should start and may keep predicting paused frames.
% \todo[inline]{BO1.21. Have we ever observed stochastic model escaping from pause state? Although it should be able to do it in theory, I haven't seen examples of this. I think that random starts are what fixes this issue.\\MB.1.22 I did observe this with SV2P.\\ LK.1.22: I did see it with SD.}

% Considering these challenges, 
In search for an effective world model we have experimented with various architectures, both new and modified versions of existing ones. In this section, we describe the architectures and the rationale behind our design decisions.  In Section \ref{sec:analysis} we compare the performance of these models.



\subsection{Deterministic Model}
Our basic architecture, presented as part of Figure~\ref{fig:full_discrete}, resembles the convolutional feedforward network from \citet{video_prediction}.  The input $X$ consists of four consecutive game frames and an action $a$. Stacked convolution layers process the visual input. The actions are one-hot-encoded and embedded in a vector which is multiplied channel-wise with the output of the convolutional layers. 
%Fully connected layers then process it and deconvolved. 
The network outputs the next frame of the game and the value of the reward.% Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

% In most of our experiments we choose the input to be four frames as with our choice of environments they fully identify the state of the game. The network is the workhorse of our simulated environment $env'$. The environment contains a memory $M$ of four frames, which is initialized with frames retrieved from the real environment. Given an action, $a$ the tuple $(M,a)$ is processed by the network outputting a new frame and a reward $r$. The oldest frame of $M$ is discarded and the new one is included. 

%\todo{pm: The next section is too much of storytelling}
%\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games.
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design, the same is true about the output $X'$.
%\todo{Important: no pooling}

In our experiments, we varied details of the architecture above. In most cases, we use a stack of four convolutional layers with $64$ filters followed by three dense layers (the first two have $1024$ neurons). The dense layers are concatenated with $64$ dimensional vector with a learnable action embedding. Next, three deconvolutional layers of $64$ filters follow. An additional deconvolutional layer outputs an image of the original $105\times 80$ size. The number of filters is either $3$ or $3 \times 256$. In the first case, the output is a real-valued approximation of pixel's RGB value. In the second case, filters are followed by softmax producing a probability distribution on the color space. The reward is predicted by a softmax attached to the last fully connected layer. 
We used dropout equal to $0.2$ and layer normalization. 

\paragraph{Loss functions.}
The visual output of our networks is either one float per pixel/channel or the categorical 256-dimensional softmax. In both cases, we used the \textit{clipped loss} $\max(Loss, C)$ for a constant $C$. We found that clipping was crucial for improving the prediction power of the models (both measured with the correct reward predictions per sequence metric and successful training using Algorithm~\ref{dpll}). We conjecture that the clipping substantially decreases the magnitude of gradients stemming from fine-tuning of big areas of background consequently letting the optimization process concentrate on small but important areas (e.g. the ball in Pong). In our experiments, we set $C=10$ for $L_2$ loss on pixel values and to $C=0.03$ for softmax loss.
Note that this means that when the level of confidence about the correct pixel value exceeds $97\%$  (as $-\ln(0.97) \approx 0.03$) we get no gradients from that pixel any longer.

\paragraph{Scheduled sampling.}
The simulator $env'$ consumes its own predictions from previous steps. Thus, due to compounding errors, the model may drift out of the area of its applicability. Following \cite{BengioVJS15}, we mitigate this problem by randomly replacing in training some frames of the input $X$ by the prediction from the previous step. Typically, we linearly increase the mixing probability during training arriving at $100\%$.

\subsection{Stochastic Models}
%In stochastic environments, explicitly modeling the stochasticity of the environment is crucial for a quality world model. Although Atari is known as a deterministic environment, it can act stochastically in practical settings. The main source of such stochasticities is the limited number of input frames as well the sprite occlusion/flickering in the observed frames. 
A stochastic model can be used to deal with limited horizon of past observed frames as well as sprites occlusion and flickering which results to higher quality predictions. 


Inspired by~\citet{sv2p}, we used a variational autoencoder ~\citep{kingma2013auto} to model the stochasticity of the environment. In this model, an additional network receives the input frames as well as the future target frame as input and approximates the distribution of the posterior. At each timestep, a latent value $z_t$ is sampled from this distribution and will be passed as input to the original predictive model. At test time, the latent values are sampled from an assumed prior 
$\mathcal{N}(\mathbf{0}, \mathbf{I})$. 
To match the assumed prior and the approximate, we use the Kullback–Leibler divergence term as an additional loss term~\citep{sv2p}.


Nonetheless, we noticed two major issues with this model. First, the weight of KL divergence loss term is game dependent and has to be optimised as a hyper-parameter which is not practical if one wants to deal with a broad portfolio of Atari games. Second, this weight is usually a very small number in the range of $[e^{-5}, e^{-3}]$ which means that the approximated posterior can diverge significantly from the assumed prior. This can result in previously unseen latent values at inference time that lead to poor predictions. We address these issues by utilizing a discrete latent variable similar to~\citet{auto_discrete}. 

As visualized in Figure~\ref{fig:full_discrete}, the proposed stochastic model with discrete latent variables discretizes the latent values into bits (zeros and ones) while training an auxiliary LSTM-based~\cite{hochreiter1997long} recurrent network to predict these bits autoregressively. At inference time, the latent bits will be generated by this auxiliary network in contrast to sampling from a prior. To make the predictive model more robust to unseen latent bits, we add uniform noise to approximated latent values before discretization and apply dropout~\cite{srivastava2014dropout} on bits after discretization.
% Already in caption: Please note that similar to~\citet{neural_discrete},
% the backpropagation bypasses the discretization operation. 
% MB: move to appendix
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{figures/model_basic_stoch.pdf}
% \caption{Architecture of stochastic model. The generative network is the same as Figure~\ref{fig:model_det} with an additional convolutional inference network to approximates the posterior given the next frame. The latent values will be sampled from approximated posterior and an assumed prior of $\mathcal{N}(\mathbf{0}, \mathbf{I})$ at training and inference time respectively.}
% \label{fig:model_stoch}
% \end{figure*}




==> SimPLe_ICRL_submission/learning_algorithm_old.tex <==
\section{Model based learning algorithm}
\label{subsec:model}

Reinforcement learning is formalized by Markov decision processes (MDP). An MDP is defined as a tuple $(\mathcal{S}, \Aa, P, r, \gamma)$, where $\mathcal{S}$ is a state space, $\Aa$ is a set of actions available to an agent, $P$ is the transition kernel, $r$ is reward function and $\gamma\in (0,1)$ is the discount factor. 

In this work we refer to MDPs as environments and assume that environments fulfill the following assumptions:
(1) Our environments do not have direct access to the state (i.e., the RAM of Atari 2600 emulator). Instead we use visual observations, typically $210\times 160$ RGB images. A single image does not determine the state. To circumvent this we stack the four previous frames. After this augmentations we will assume that the observation can be identified with the state.
%%SL.1.15: can probably remove that last sentence -- since the model is recurrent anyway, I'm not sure we even need this assumption
(2) Our environments are deterministic, namely the transition kernel $P$ can be identified with a function $env:\mathcal{S}\times \Aa\mapsto \mathcal{S}$, i.e. given a state and action the environment produces the next state.
%%SL.1.15: do we actually need this assumption?
(3) The action space $\Aa$ and the space of rewards are finite. 

A reinforcement learning agent interacts with the MDP issuing actions according to a policy. Formally, policy $\pi$ is a mapping from states to probability distributions over $\mathcal{A}$. The quality of a policy is measured by the value function $\mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s_0=s \right)$, which for a starting state $s$ estimates the total discounted reward gathered by the agent. In Atari 2600 games our goal is to find a policy which maximizes the value function when the starting state is the beginning of the game.

Crucially, apart from a Atari 2600 emulator environment $env$ we will use \textit{a neural network simulated environment} $env'$. The environment $env'$ shares the action and reward spaces with $env$ and produces visual observations in the same format. The  environment $env'$ will be trained to mimic $env$.  The principal aim of our work is to check
%%SL.1.15: well, maybe not just to check -- perhaps we can say The principal aim of our work is to train a policy...
if one can 
train a policy $\pi$ using a simulated environment $env'$ so that $\pi$ achieves a desired performance in the original environment $env$. During the training we aim to use as little interactions with $env$ as possible. 


The initial data to train $env'$ comes from random rollouts of $env$. As this is unlikely to capture all aspects of the environment, thus we use the following data-aggregation iterative algorithm inspired by Section 4 in  \cite{trpo_ensemble} and Section 5 in \cite{world_models}.
%%SL.1.15: To be fair, this basic scheme has been in use for decades and is basically ubiquitous for model-based RL. Feels odd to credit it to two papers from the last couple of years.

%\begin{figure*}[H]
\begin{algorithm}[H]
\caption{Pseudocode for model-based RL}\label{dpll}
\begin{algorithmic}
\STATE Initialize policy $\boldsymbol\pi$
\STATE Initialize model parameters $env'$
\STATE Initialize empty set $\mathbf{D}$
\WHILE{not done} 
\STATE \underline{$\triangleright$ collect observations from real env.}
\WHILE{not enough observations}
\STATE $(\mathbf{state},\mathbf{reward}) \gets env(\boldsymbol\pi(\mathbf{state}))$
\STATE $\mathbf{D} \gets \mathbf{D} \cup (\mathbf{state},\mathbf{reward})$
\ENDWHILE
\STATE \underline{$\triangleright$ update model using collected data.}
\STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env`, \mathbf{D})$
\STATE \underline{$\triangleright$ update policy using world model.}
\STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, \boldsymbol\theta)$
\ENDWHILE
\end{algorithmic}
\label{basic_loop}
\label{alg:basic_loop}
\end{algorithm}
% \end{figure*}

==> SimPLe_ICRL_submission/learning_algorithm_old_v2.tex <==
\section{Model based learning algorithm}
\label{subsec:model}

Reinforcement learning is formalized by Markov decision processes (MDP). An MDP is defined as a tuple $(\mathcal{S}, \Aa, P, r, \gamma)$, where $\mathcal{S}$ is a state space, $\Aa$ is a set of actions available to an agent, $P$ is the transition kernel, $r$ is reward function and $\gamma\in (0,1)$ is the discount factor. 

In this work we refer to MDPs as environments and assume % that environments fulfill the following assumptions:
that environments do not have direct access to the state (i.e., the RAM of Atari 2600 emulator). Instead we use visual observations, typically $210\times 160$ RGB images. A single image does not determine the state. To circumvent this we stack the four previous frames.
% \todo[inline]{BO.1.21: Maybe it would be worth to add a footnote explaining that four previous frames is not always sufficient to capture the state? Or have a section on this in latter chapter and here just refer to it?}
%5(2) Our environments are deterministic, namely the transition kernel $P$ can be identified with a function $env:\mathcal{S}\times \Aa\mapsto \mathcal{S}$, i.e. given a state and action the environment produces the next state.
% \todo[inline]{LK.1.22: I think we don't need this assumption as we're using stochastic models now, right? Can we remove it?}
%%SL.1.15: do we actually need this assumption?
(3) The action space $\Aa$ and the space of rewards are finite. 

A reinforcement learning agent interacts with the MDP issuing actions according to a policy. Formally, policy $\pi$ is a mapping from states to probability distributions over $\mathcal{A}$. The quality of a policy is measured by the value function $\mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s_0=s \right)$, which for a starting state $s$ estimates the total discounted reward gathered by the agent. In Atari 2600 games our goal is to find a policy which maximizes the value function when the starting state is the beginning of the game.

Crucially, apart from a Atari 2600 emulator environment $env$ we will use \textit{a neural network simulated environment} $env'$. The environment $env'$ shares the action and reward spaces with $env$ and produces visual observations in the same format. The  environment $env'$ will be trained to mimic $env$.  The principal aim of our work is to
train a policy $\pi$ using a simulated environment $env'$ so that $\pi$ achieves a desired performance in the original environment $env$. During the training we aim to use as few interactions with $env$ as possible. 


The initial data to train $env'$ comes from random rollouts of $env$. As this is unlikely to capture all aspects of the environment, thus we use the data-aggregation iterative algorithm presented in Algorithm~\ref{alg:basic_loop}.
\begin{figure}
\removelatexerror
\begin{algorithm}[H]
\caption{Pseudocode for model-based RL}\label{dpll}
\begin{algorithmic}
\STATE Initialize policy $\boldsymbol\pi$
\STATE Initialize model parameters $env'$
\STATE Initialize empty set $\mathbf{D}$
\WHILE{not done} 
\STATE \underline{$\triangleright$ collect observations from real env.}
\WHILE{not enough observations}
\STATE $(\mathbf{state},\mathbf{reward}) \gets env(\boldsymbol\pi(\mathbf{state}))$
\STATE $\mathbf{D} \gets \mathbf{D} \cup (\mathbf{state},\mathbf{reward})$
\ENDWHILE
\STATE \underline{$\triangleright$ update model using collected data.}
\STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env`, \mathbf{D})$
\STATE \underline{$\triangleright$ update policy using world model.}
\STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, \boldsymbol\theta)$
\ENDWHILE
\end{algorithmic}
\label{basic_loop}
\label{alg:basic_loop}
\end{algorithm}
\end{figure}

==> SimPLe_ICRL_submission/learning_alogrithm.tex <==
\section{Simulated Policy Learning (SimPLe)}
\label{subsec:model}
\label{sec:mbrl}

% TODO_PM_21_05. Shorter version:
% Reinforcement learning is concerned with sequential decision-making problems. Given an \textit{environment}, which changes its \textit{state} and provides \textit{rewards} based on the performed \textit{actions}, the goal is to find an optimal behavior (\textit{policy} $\pi$) of an agent, which based on the current observation from the environment performs an appropriate action to maximize the discounted sum of future rewards.

% In this work we focus on Atari games, which provide visual observations of the current game screen. Because this image does not convey the full state of the environment, we stack the four last frames to provide richer input to the agent.

% Our method, apart from an Atari 2600 emulator environment $env$, uses \textit{a neural network simulated environment} $env'$ which we call a \textit{world model}, trained to mimic dynamics of $env$. Our principal aim is to train a policy $\pi$ using the simulated environment $env'$ so that $\pi$ achieves good performance in the original environment $env$. In our training process, summarized in Algorithm~\ref{alg:basic_loop}, we aim to use as few interactions with $env$ as possible. As this is unlikely to capture all aspects of the environment, we use an iterative data-aggregation method consisting of collecting data from $env$ using the policy, training the model $env'$ on the collected data and training the policy using $env'$. 

% \begin{figure}  % \small
% \removelatexerror
% \begin{algorithm}[H]
% \caption{Pseudocode for SimPLe}\label{dpll}
% \begin{algorithmic}
% \STATE Initialize policy $\boldsymbol\pi$, 
%   model parameters $env'$, $\mathbf{D} = \emptyset$
% \WHILE{not done} 
% \STATE \underline{$\triangleright$ collect observations from real env.}
% \WHILE{not enough observations}
% \STATE $a \gets \boldsymbol\pi(s)$
% \STATE $(s' ,r) \gets env(a)$
% \STATE $\mathbf{D} \gets \mathbf{D} \cup (s,a,r,s')$
% \STATE $s \leftarrow s'$
% \ENDWHILE
% \STATE \underline{$\triangleright$ update model using collected data.}
% \STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env', \mathbf{D})$
% \STATE \underline{$\triangleright$ update policy using world model.}
% \STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, \boldsymbol\theta)$
% \ENDWHILE
% \end{algorithmic}
% \label{basic_loop}
% \label{alg:basic_loop}
% \end{algorithm}
% \end{figure}

Reinforcement learning is formalized in Markov decision processes (MDP). An MDP is defined as a tuple $(\mathcal{S}, \Aa, P, r, \gamma)$, where $\mathcal{S}$ is a state space, $\Aa$ is a set of actions available to an agent, $P$ is the unknown transition kernel, $r$ is the reward function and $\gamma\in (0,1)$ is the discount factor. 
In this work we refer to MDPs as environments and assume % that environments fulfill the following assumptions:
that environments do not provide direct access to the state (i.e., the RAM of Atari 2600 emulator). Instead we use visual observations, typically $210\times 160$ RGB images. A single image does not determine the state. 
% This is still observation not state.
In order to reduce environment's partial observability, we stack four consecutive frames and use it as the observation.
A reinforcement learning agent interacts with the MDP by issuing actions according to a policy. Formally, policy $\pi$ is a mapping from states to probability distributions over $\mathcal{A}$. The quality of a policy is measured by the value function $\mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s_0=s \right)$, which for a starting state $s$ estimates the total discounted reward gathered by the agent.

\begin{wrapfigure}[14]{r}{0.45\textwidth}
\removelatexerror
\vspace{-0.5cm}
\begin{algorithm}[H]
\caption{Pseudocode for SimPLe}\label{dpll}
\begin{algorithmic}
\STATE Initialize policy $\boldsymbol\pi$
\STATE Initialize model parameters $\boldsymbol\theta$ of $env'$
\STATE Initialize empty set $\mathbf{D}$
\WHILE{not done} 
\STATE \underline{$\triangleright$ collect observations from real env.}
\STATE $\mathbf{D} \gets \mathbf{D} \cup \text{COLLECT($env$, $\pi$)}$
\STATE \underline{$\triangleright$ update model using collected data.}
\STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env', \mathbf{D})$
\STATE \underline{$\triangleright$ update policy using world model.}
\STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, env')$
\ENDWHILE
\end{algorithmic}
\label{basic_loop}
\label{alg:basic_loop}
\end{algorithm}
%\vspace{-0.8cm}
\end{wrapfigure}

In Atari 2600 games our goal is to find a policy which maximizes the value function from the beginning of the game.
Crucially, apart from an Atari 2600 emulator environment $env$ we will use \textit{a neural network simulated environment} $env'$ which we call a \textit{world model} and describe in detail in Section \ref{sec:world_models}. The environment $env'$ shares the action space and reward space with $env$ and produces visual observations in the same format, as it will be trained to mimic $env$.  Our principal aim is to
train a policy $\pi$ using a simulated environment $env'$ so that $\pi$ achieves good performance in the original environment $env$. In this training process we aim to use as few interactions with $env$ as possible. 
The initial data to train $env'$ comes from random rollouts of $env$. As this is unlikely to capture all aspects of $env$, we use the iterative method presented in Algorithm~\ref{alg:basic_loop}.

==> SimPLe_ICRL_submission/macros.tex <==

% if you need to pass options to natbib, use, e.g.:
% \PassOptionsToPackage{numbers, compress}{natbib}
% before loading nips_2018

% ready for submission
% \usepackage{nips_2018}

% to compile a preprint version, e.g., for submission to arXiv, add
% add the [preprint] option:
% \usepackage[preprint]{nips_2018}

% to compile a camera-ready version, add the [final] option, e.g.:
% \usepackage[final]{nips_2018}

% to avoid loading the natbib package, add option nonatbib:
% \usepackage[nonatbib]{nips_2018}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage[colorlinks=true, linkcolor=black, citecolor=black, filecolor=black, urlcolor=black]{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{amsmath}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

% \usepackage{algorithm2e}
% \usepackage[noend]{algpseudocode}
\usepackage[ruled, vlined, linesnumbered]{algorithm2e}
% \algsetup{linenosize=\small}
% \usepackage{etoolbox}\AtBeginEnvironment{algorithm}{\small}

\usepackage{todonotes}

\newcommand{\env}{{\texttt{env}}}
\newcommand{\Env}{{\texttt{Env}}}
\newcommand{\Aa}{{\mathcal A}}
\newcommand{\Rr}{{\mathcal R}}
\newcommand{\Oo}{{\mathcal O}}
\newcommand{\Dd}{{\mathcal D}}
\newcommand{\Prob}{{\mathcal P}}

\newcommand{\pong}{\texttt{Pong}}
\newcommand{\breakout}{\texttt{Breakout}}
\newcommand{\freeway}{\texttt{Freeway}}
\newcommand{\bankh}{\texttt{Bank Heist}}
\newcommand{\boxing}{\texttt{Boxing}}
\newcommand{\bowling}{\texttt{Bowling}}
\newcommand{\asterix}{\texttt{Asterix}}
\newcommand{\seaquest}{\texttt{Seaquest}}
\newcommand{\hero}{\texttt{Hero}}
\newcommand{\crazyclimber}{\texttt{Crazy Climber}}
\newcommand{\kungfumaster}{\texttt{Kung Fu Master}}
\newcommand{\atlantis}{\texttt{Atlantis}}
\newcommand{\battlezone}{\texttt{Battle Zone}}
\newcommand{\privateeye}{\texttt{Private Eye}}


\usepackage[font={footnotesize,it}]{caption}

\newtheorem{definition}{Definition}

\usetikzlibrary{shapes.geometric,backgrounds,
  positioning-plus,node-families,calc}
\tikzset{
  basic box/.style = {
    shape = rectangle,
    align = center,
    draw  = #1,
    fill  = #1!25,
    rounded corners},
  header node/.style = {
    Minimum Width = header nodes,
    font          = \strut\Large\ttfamily,
    text depth    = +0pt,
    fill          = white,
    draw},
  header/.style = {%
    inner ysep = +1.5em,
    append after command = {
      \pgfextra{\let\TikZlastnode\tikzlastnode}
      node [header node] (header-\TikZlastnode) at (\TikZlastnode.north) {#1}
      node [span = (\TikZlastnode)(header-\TikZlastnode)]
        at (fit bounding box) (h-\TikZlastnode) {}
    }
  },
  hv/.style = {to path = {-|(\tikztotarget)\tikztonodes}},
  vh/.style = {to path = {|-(\tikztotarget)\tikztonodes}},
  fat blue line/.style = {ultra thick, blue}
}

\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,positioning}

\definecolor{echoreg}{HTML}{2cb1e1}
\definecolor{olivegreen}{rgb}{0,0.6,0}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\usepackage{etoolbox}

\newtoggle{redraw}
\newtoggle{redraw2}

\usepackage{wrapfig}

\tikzset{%
pics/cube/.style args={#1/#2/#3/#4}{code={%
	\begin{scope}[line width=#4mm]
	\begin{scope}
	\clip (-#1,-#2,0) -- (#1,-#2,0) -- (#1,#2,0) -- (-#1,#2,0) -- cycle;
	\filldraw (-#1,-#2,0) -- (#1,-#2,0) -- (#1,#2,0) -- (-#1,#2,0) -- cycle;
	\end{scope}
\iftoggle{redraw}{%
}{%
	\begin{scope}
	\clip (-#1,-#2,0) -- (-#1-#3,-#2,-#3) -- (-#1-#3,#2,-#3) -- (-#1,#2,0) -- cycle;
	\filldraw (-#1,-#2,0) -- (-#1-#3,-#2,-#3) -- (-#1-#3,#2,-#3) -- (-#1,#2,0) -- cycle;
	\end{scope}
}
\iftoggle{redraw2}{%
}{
	\begin{scope}
	\clip (-#1,#2,0) -- (-#1-#3,#2,-#3) -- (#1-#3,#2,-#3) -- (#1,#2,0) -- cycle;
	\filldraw (-#1,#2,0) -- (-#1-#3,#2,-#3) -- (#1-#3,#2,-#3) -- (#1,#2,0) -- cycle;
	\end{scope}
}
	\node[inner sep=0] (-A) at (-#1-#3*0.5, 0, -#3*0.5) {};
	\node[inner sep=0] (-B) at (#1-#3*0.5, 0, -#3*0.5) {};
	
	\coordinate (-V) at (#1, #2);
	\coordinate (-W) at (#1, -#2);
	\end{scope}
}}}

% macros for recurrent simulators

\usepackage{amsmath}

\renewcommand{\figref}[1]{Fig. \ref{#1}}
\renewcommand{\secref}[1]{Sec. \ref{#1}}
\newcommand{\appref}[1]{Appendix \ref{#1}}
\definecolor{myred}{cmyk}{0,0.9,0.9,0.1}
\definecolor{myblue}{cmyk}{0,0.3,0.9,0.1}
\newcommand{\myred}{\color{myred}}
\newcommand{\myblue}{\color{myblue}}
\newcommand{\PDT}{PDT}
\newcommand{\ODT}{ODT}
\newcommand{\OD}{observation-dependent} 
\newcommand{\PD}{prediction-dependent} 
\setlength{\bibsep}{0.2pt}

\newcommand{\myvec}[1]{\mathbf{#1}}
\renewcommand{\va}{\myvec{a}}
\renewcommand{\vc}{\myvec{c}}
\renewcommand{\vf}{\myvec{f}}
\renewcommand{\vh}{\myvec{h}}
\renewcommand{\vi}{\myvec{i}}
\renewcommand{\vo}{\myvec{o}}
\renewcommand{\vs}{\myvec{s}}
\renewcommand{\vv}{\myvec{v}}
\renewcommand{\vx}{\myvec{x}}
\renewcommand{\vy}{\myvec{y}}
\renewcommand{\vz}{\myvec{z}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\ha}{\vv}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\ie}{\emph{i.e.}}
\newcommand{\eg}{\emph{e.g.}}


%\usepackage{caption}
% \captionsetup{font=footnotesize}

\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother

==> SimPLe_ICRL_submission/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> SimPLe_ICRL_submission/pm_introduction.tex <==
\section{Introduction}

Human players can learn to play Atari games in minutes~\citep{human_atari_minutes}. However, some of the best model-free reinforcement learning algorithms require tens or hundreds of millions of time steps -- the equivalent of several weeks of training in real time. How is it that humans can learn these games so much faster? Perhaps part of the puzzle is that humans possess an intuitive understanding of the physical processes that are represented in the game: we know that planes can fly, balls can roll, and bullets can destroy aliens. We can therefore predict the outcomes of our actions. In this paper, we explore how learned video models can enable learning in the Atari Learning Environment (ALE) benchmark~\cite{ale, ale2} with a budget restricted to 100K time steps -- roughly to two hours of a play time.

Although prior works have proposed training predictive models for next-frame, future-frame, as well as combined future-frame and reward predictions in Atari games (\cite{video_prediction,recurrent, video_reward_prediction}), no prior work has successfully demonstrated model-based control via predictive models that achieve competitive results with model-free RL. Indeed, in a recent survey (Section 7.2 in \citet{ale2}) this was formulated as the following challenge: ``\emph{So far, there has been no clear demonstration of successful planning with a learned model in the ALE}''.


Using models of environments, or informally giving the agent ability to predict its future, has a fundamental appeal for reinforcement learning. The spectrum of possible applications is vast, including learning policies
from the model \citep[Chapter~8]{embed_to_control, deep_spatial, finn2016, ebert, hafner, piergiovanni, rybkin-pertsch,sutton_barto_2017}, capturing important details of the scene \citep{world_models}, encouraging exploration \citep{video_prediction},  creating intrinsic motivation \citep{schmidhuber_formal_theory} or counterfactual reasoning \citep{woulda_coulda_shoulda}.
One of the exciting benefits of model-based learning is the promise to substantially improve sample efficiency of deep reinforcement learning (see Chapter~8 in \cite{sutton_barto_2017}).

Our work advances the state-of-the-art in model-based reinforcement learning by introducing a system that, to our knowledge, is the first to successfully handle a variety of challenging games in the ALE benchmark. To that end, we experiment with several stochastic video prediction techniques, including a novel model based on discrete latent variables. We present an approach, called Simulated Policy Learning (SimPLe), that utilizes these video prediction techniques and trains a policy to play the game within the learned model. With several iterations of dataset aggregation, where the policy is deployed to collect more data in the original game, we learn a policy that, for many games, successfully plays the game in the real environment (see videos on the project webpage \url{https://goo.gl/itykP8}). %\href{https://sites.google.com/view/modelbasedrlatari/home}{dedicated webpage\footnote{\url{https://sites.google.com/view/modelbasedrlatari/home}} with visualizations} of experiments presented in Section \ref{sec:experiments}). 

In our empirical evaluation, we find that SimPLe is significantly more sample-efficient than a highly tuned version of the state-of-the-art Rainbow algorithm~\citep{rainbow} on almost all games. In particular, in low data regime of $100$k samples, on more than half of the games, our method achieves a score which Rainbow requires at least twice as many samples. In the best case of {\freeway}, our method is more than 10x more sample-efficient, see Figure \ref{fig:compare_dopamine_ppo}.
% BO 2020/02/12.
Since the publication of the first preprint of this work, it has been shown in \cite{nips/HasseltHA19, kielak2020do} that Rainbow can be tuned to have better results in low data regime. The results are on a par with SimPLe -- both of the model-free methods are better in 13 games, while SimPLe is better in the other 13 out of the total 26 games tested (note that in Section 4.2 \cite{nips/HasseltHA19} compares with the results of our first preprint, later improved). 

\begin{figure}
\centering
\includegraphics[width=0.75\textwidth]{figures/Cycle_full.png}
\caption{Main loop of SimPLe. 1) the agent starts interacting with the real environment following the latest policy (initialized to random). 2) the collected observations will be used to train (update) the current world model. 3) the agent updates the policy by acting inside the world model. The new policy will be evaluated to measure the performance of the agent as well as collecting more data (back to 1).  Note that world model training is self-supervised for the observed states and supervised for the reward.} 
\label{fig:main_cycle}
\vspace{-0.4cm}
\end{figure}


==> SimPLe_ICRL_submission/policies.tex <==
\section{Policy Training} \label{sec:policy_training}

%TODO_PM_21_05: Possibly use the short version below and move the current text to the appendix.
% To train the policy (TRAIN\_RL in Algorithm \ref{alg:basic_loop}) we use the proximal policy optimization (PPO) algorithm~\cite{ppo}. It generates rollouts using the simulated environment $env'$ and uses them to improve the policy $\pi$. The fundamental difficulty lays in imperfections of the model compounding over time. To mitigate this problem we use short rollouts of $env'$ starting from ground-truth frames sampled from the buffer $D$. End of such rollout is not treated as end of episode in policy learning - the value estimate provided by PPO is used to mimic the following rewards. 

% We stress that imperfections in the model are unavoidable, as it is trained using only data generated with the current policy. For this reason in Algorithm~\ref{alg:basic_loop} we collect data iteratively, using the newest policy in each loop's COLLECT.

We will now describe the details of SimPLe, outlined in Algorithm \ref{alg:basic_loop}.  In step 6 we use the proximal policy optimization (PPO) algorithm~\citep{ppo} with $\gamma=0.95$. The algorithm generates rollouts in the simulated environment $env'$ and uses them to improve policy $\pi$. The fundamental difficulty lays in imperfections of the model compounding over time. To mitigate this problem we use short rollouts of $env'$. Typically every $N=50$ steps we uniformly sample the starting state from the ground-truth buffer $D$ and restart $env'$ (for experiments with the value
of $\gamma$ and $N$ see Section~\ref{subabl}). Using short rollouts may have a degrading effect as the PPO algorithm does not have a way to infer effects longer than the rollout length. To ease this problem, in the last step of a rollout we add to the reward the evaluation of the value function.
% Isn't this present in the standard PPO as well?
Training with multiple iterations re-starting from trajectories gathered in the real environment is  new to our knowledge. It was inspired by the classical Dyna-Q algorithm and, notably, in the Atari domain no comparable results have been achieved.

%We stress that imperfections in the model are unavoidable, as the model is trained using only data generated with the current policy. Moreover, the training of the world model is prone to overfitting as we try to gather as little data as possible from the real environment. Finally, sometimes the model fails in a catastrophic way by losing semantic coherence (e.g., a disappearing ball in Pong). 

The main loop in Algorithm \ref{dpll} is iterated $15$ times (cf. Section~\ref{subabl}). The world model is trained for $45$K steps in the first iteration and for $15$K steps in each of the following ones.  Shorter training in later iterations does not degrade the performance because the world model after first iteration captures already part of the game dynamics and only needs to be extended to novel situations.

In each of the iterations, the agent is trained inside the latest world model using PPO. In every PPO epoch we used 16 parallel agents collecting 25, 50 or 100 steps from the simulated environment $env'$ (see Section \ref{subabl} for ablations). The number of PPO epochs is $z\cdot 1000$, where $z$ equals to 1 in all passes except last one (where $z = 3$) and two passes number 8 and 12 (where $z = 2$). This gives $800$K$\cdot z$ interactions with the simulated environment in each of the loop passes. In the process of training the agent performs  $15.2$M interactions with the simulated environment $env'$.


==> SimPLe_ICRL_submission/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

Atari games gained prominence as a benchmark for reinforcement learning with the introduction of the Arcade Learning Environment (ALE)~\cite{ale}. The combination of reinforcement learning and deep models then enabled RL algorithms to learn to play Atari games directly from images of the game screen, using variants of the DQN algorithm~\citep{dqn, dqn2, rainbow} and actor-critic algorithms~\citep{a3c,ppo,ga3c,acktr,vtrace}.
% An interesting approach has been proposed in Sodhani 2019, where learning a consistent model helps to train policies that are more powerful than model-free baseline A2C.
The most successful methods in this domain remain model-free algorithms~\citep{rainbow,vtrace}. Although the sample complexity of these methods has substantially improved recently, it remains far higher than the amount of experience required for human players to learn each game~\citep{human_atari_minutes}. In this work, we aim to learn Atari games with a budget of just 100K agent steps (400K frames), corresponding to about two hours of play time. Prior methods are generally not evaluated in this regime, and we therefore optimized Rainbow~\citep{rainbow} for optimal performance on 1M steps, see Appendix \ref{sec:baselines_optimizations} for details.

\citet{video_prediction} and \citet{recurrent} show that learning predictive models of Atari 2600 environments is possible using appropriately chosen deep learning architectures. Impressively, in some cases the predictions maintain low $L_2$ error over timespans of hundreds of steps. 
As learned simulators of Atari environments are core ingredients of our approach, in many aspects our work is motivated by \citet{video_prediction} and \citet{recurrent}, however we focus on using video prediction in the context of learning how to play the game well and positively verify that learned simulators can be used to train a policy useful in original environments.
An important step in this direction was made by \citet{video_reward_prediction}, which extends the work of \citet{video_prediction} by including reward prediction, but does not use the model to learn policies that play the games.
Most of these approaches, including ours, encode knowledge of the game in implicit way. Unlike this, there are works in which modeling is more explicit, for example \cite{ersen2014learning} uses testbed of the Incredible Machines to learn objects behaviors and their interactions.
Similarly \citet{guzdial2017game} learns an engine predicting interactions of predefined set of sprites in the domain of Super Mario Bros.

Perhaps surprisingly, there is virtually no work on model-based RL in video games from images.
Notable exceptions are the works of
\citet{vpn}, \citet{sodhani2019learning}, \citet{world_models}, \citet{dyna_dqn}, \cite{leibfried2018model} and \citet{gats}. \citet{vpn} use a model of rewards to augment model-free learning with good results on a number of Atari games. However, this method does not actually aim to model or predict future frames, and achieves clear but relatively modest gains in efficiency.
\citet{sodhani2019learning} proposes learning a model consistent with RNN policy which helps to train policies that are more powerful than their model-free baseline.
\citet{world_models} present a way to compose a variational autoencoder with a recurrent neural network into an architecture  
that is successfully evaluated in the VizDoom environment and on a 2D racing game. The training procedure is similar to  Algorithm \ref{alg:basic_loop}, but only one iteration of the loop is needed as the environments are simple enough to be fully explored with random exploration. Similarly, \citet{alaniz2018deep} utilizes a transition model with Monte Carlo tree search to solve a block-placing task in Minecraft. \citet{dyna_dqn} use a variant of Dyna~\citep{dyna} to learn a model of the environment and generate experience for policy training in the context of Atari games. Using six Atari games as a benchmark \citet{dyna_dqn} measure the impact of planning shapes on performance of the Dyna-DQN algorithm and include ablations comparing scores obtained with perfect and imperfect models. Our method achieves around 330\% of the Dyna-DQN score on Asterix, 120\% on Q-Bert, 150\% on Seaquest and 80\% on Ms. Pac-Man. \cite{gats} propose an algorithm called Generative Adversarial Tree Search (GATS) and for five Atari games train a GAN-based world model along with a Q-function. \cite{gats} primarily discuss various failure modes of the GATS algorithm. Our method achieves around 64 times the score of GATS on Pong and 10 times on Breakout. \footnote{Comparison with Dyna-DQN and GATS is based on  random-normalized scores achieved at 100K interactions. Those are approximate, as the authors Dyna-DQN and GATS have not provided tabular results. Authors of Dyna-DQN also report scores on two games which we do not consider: Beam Rider and Space Invaders. For both games the reported scores are close to random scores, as are GATS scores on Asterix.}

Outside of games, model-based reinforcement learning has been investigated at length for applications such as robotics~\citep{deisenroth}. Though most of such works do not use image observations, several recent works
have incorporated images into real-world~\citep{deep_spatial, finn2016, sv2p, ebert, piergiovanni, paxton, rybkin-pertsch, ebert2018visual} and simulated~\citep{embed_to_control, hafner} robotic control. 
%
Our video models of Atari environments described in Section \ref{sec:architectures} are motivated by models developed in the context of robotics. Another source of inspiration are discrete autoencoders proposed by \citet{neural_discrete} and \citet{auto_discrete}.

The structure of the model-based RL algorithm that we employ consists of alternating between learning a model, and then using this model to optimize a policy with model-free reinforcement learning. Variants of this basic algorithm have been proposed in a number of prior works, starting from Dyna~Q \cite{dyna} to more recent methods that incorporate deep networks
\cite{stochastic_value_gradients, model_based_value_estimation, uncertainty_driven_imagination, trpo_ensemble}. 

==> SimPLe_ICRL_submission/related_work_old.tex <==
\section{Related work}
\label{sec:related_work}

% \paragraph{Model-free algorithms and Atari games.} 
In \cite{dqn} the authors presented the DQN algorithm which learns to play a large number of Atari games. The algorithm was extended in \cite{ppo,acktr,dqn2,rainbow,a3c} towards higher performance and better parallelization. % and in \cite{acktr} towards sample efficiency. % \todo[inline]{Add more "sample efficient" methods?} % emphasizes sample efficiency and in a number of games achieves the state-of-the-art performance utilizing only 2 million frames. Other above mentioned algorithms tend to utilize at least an order of magnitude more frames to achieve the top performance. 
%%SL.12.27:  Maybe it would be good to put this paragraph first in this section, as a way to motivate and set up the problem? That would then flow nicely into model-based RL, where the end of this paragraph can state clearly the model-free RL challenges.
In this work we are addressing a question what kind of performance in Atari games can be achieved within the budget of 100K frames. None of the above methods was tested against such a strict sample efficiency requirement, hence in this work we include a thorough evaluation of the PPO \cite{ppo} and Rainbow \cite{rainbow} algorithms optimized for performance on 100K and 1M frames, see Table \ref{table:rainbow}.

% \paragraph{Model-based methods.}  
% The budget of 100K frames is spent on learning of the model of environment.  
In \cite{recurrent,video_prediction} it is shown that learning of Atari 2600 environments is possible using appropriately chosen deep learning architectures. Impressively, in some cases the predictions maintain high $L_2$ accuracy over timespans of hundreds steps. % Learning of rewards is not reported.
%%SL.12.27: I understand why that last sentence is important, but it feels somehow passive aggressive. Maybe we can just remove it and make everyone happier?
%%CF.12.27: What we could do is later phrase that, unlike prior work, we focus on using video prediction in the context of learning the play the game well.
As learned simulators of Atari environments are core ingredients of our approach, in many aspects our work is motivated by \cite{recurrent,video_prediction}, however we focus on using video prediction in the context of learning how to play the game well and positively verify that learned simulators can be used to train a policy useful in original environments. In other terms we are making a step from a pure video-prediction task in \cite{recurrent,video_prediction} to a model-based learning for Atari games. 
Perhaps surprisingly, there is virtually no work on model-based learning in video games. A notable exception is 
%an interesting new work 
\cite{world_models}. The authors compose variational autoencoders with recurrent neural networks into an architecture being able to model evolution of non-deterministic games. This architecture is successfully evaluated in the VizDoom environment on a task which requires avoiding random fireballs. They propose a training procedure, which is essentially the same as Algorithm \ref{alg:basic_loop}. In the VizDoom experiment they need only one loop as the environment has rather dense rewards and is simple enough to be discovered by random exploration. % Interestingly, they increase the randomness of the simulator to prevent training from exploiting loopholes of the neural network model.

For a survey of model-based methods for robotics see \cite[Chapter 3]{deisenroth}. In this domain recent works  \cite{finn2016, ebert, hafner, piergiovanni, paxton, rybkin-pertsch}  are focused on learning models from raw pixels and our approach to learning of models in Atari games is closely motivated by this line of research, see Section \ref{sec:architectures} for detailed description of our models used for video and reward predictions.  Another source of motivation is a stochastic video prediction model \cite{sv2p} and discrete autoencoders described in \cite{neural_discrete, auto_discrete}.   % In \cite{trpo_ensemble} the model-based approach is applied in the context of the MuJoCo physics simulator \cite{mujoco}. 

In a recent work \cite{trpo_ensemble} a training loop similar to one described in  Algorithm \ref{basic_loop} along with a policy gradient algorithm \cite{trpo} was applied to a number of robotic tasks in the MuJoCo physics simulator \cite{mujoco}. Learning in  \cite{trpo_ensemble} is based on the state of the robot and does not involve visual inputs. 

% \paragraph{Augmenting model-free reinforcement learning using a model.} In \cite{imagination_metacontrol,imagination_model_based_planning} a model of the environment called {\em imagination} is used to augment performance of a model-free reinforcement learning algorithm. This proved to be particularly useful in games like Sokoban, where certain moves are irreversible. 
% HM.1.9:  removing imagination to save space, also it does not involve Atari

%There are number of differences though. We argue that the $L_2$ accuracy is not necessarily a good proxy measure for assessing applicability in reinforcement learning. Instead we argue for using \textit{correct rewards per sequence} metric (see Section \ref{sec:architectures}). In fact we found that training models with poor $L_2$ accuracy might be beneficial for \textit{correct rewards per sequence} metric as explained in Section \ref{sec:architectures}.
%%SL.12.27: I think this statement perhaps places somewhat undue emphasis on the metric. I can see the importance, but coming this early in the paper, readers might misunderstand it as suggesting that this is the key component that makes the method work at all...
% Finally, we positively verify that our simulations can be used to train a policy useful in original environments. 
% \paragraph{Learning models from pixels.} In \cite{pixel1, pixel2, pixel3, raw_visual}
%%SL.12.27: the first two are not concerned with robotics, the third one is robotics but doesn't learn models on pixels, and the fourth one is on pixels but doesn't learn models :) Chelsea can probably suggest the right related work to put here, but maybe what I might suggest is to first have a block of citations about model-based RL in general (whether from pixels or not), and cite the Deisenroth survey paper there, and then have a block of citations on learning models from pixels and cite papers that do that all together (Chelsea can probably provide this list)
%%CF.12.27: The relevant citations for model-based RL with raw pixel input is:
% -- Learn autoencoder on pixels and learn model in latent space: embed to control (Watter et al), deep spatial autoencoders (Finn et al), Danijar Hafner's latest paper (https://arxiv.org/abs/1811.04551)
% -- Learn model in pixel space and use it for planning and control: deep visual foresight (Finn et al.), self-supervised visual planning (Ebert et al), 
% -- this paper: https://arxiv.org/abs/1806.09655
% -- this paper: https://arxiv.org/abs/1805.07813
% -- this paper: https://arxiv.org/abs/1804.00062 (trains video predictor on demonstrations, not on autonomously collected data, so not really doing model-based RL, but still using video prediction)
% the model-based approach is applied to robotics. Models are taking images as inputs and  policies are trained to perform tasks such as moving a robotic arm or grasping of an object. In this work we focus on Atari games. This  standard reinforcement learning benchmark allows for an easy comparison of obtained results with the state-of-the-art achieved by model-free reinforcement learning algorithms.

% \paragraph{Learning of models in other games.} 
%%SL.12.27: I feel like we are better off having a more general discussion of related work on model-based reinforcement learning from pixels and adding this paper as one of the citations -- there are plenty of papers that do essentially the same thing, so it feels weird to single it out for an entire paragraph just because it's from Google (or for any other reason). For example, the e2c paper also uses VAEs.
%%CF.12.27: I agree that it doesn't make sense to separate this from the papers above. It belongs in the same category as embed-to-control/E2C, which I mentioned above.
%%HM.6.01: I agree with the criticism to some extend and will attempt to re-write it, but the main reason why it occupies so much space is that we are doing video games and the cited paper is the only one which also does video games. Besides, when we have started to talk with LK about the current project in Nov 2017, LK was aware of progress and of limitations of David's project and our work was intended to address some of these limitations. 

% \paragraph{Learning models from the state of a physics simulator.} In \cite{trpo_ensemble, mpc_model_based} the model-based approach is applied in the context of the MuJoCo physics simulator \cite{mujoco}. The simulator exposes the state of the environment which is in practice a vector of floats of length up to $50$. Authors of \cite{trpo_ensemble, mpc_model_based} use a data collection method similar to the one described in Algorithm \ref{basic_loop}.
%%SL.12.27: there are something like three decades of research on model-based RL algorithms... maybe a better scoping for related work would be to just cite the deisenroth survey and a couple recent papers (first) and then mostly focus on the pixel-based methods?

%(the latter has a good bibliography review for robotics)
%Missing bibliography \todo[inline]{Include the work on MuJoCo into the bibliography - they are in a separated model-based doc https://docs.google.com/document/d/1rjLmIoAGINii97cUCkSPcse61veQqd27wzEoOmL-Etc/edit?usp=sharing }
%%HM 6.01 trpo_ensemble has a unique (?) feature that iterated TRPO is used to learn policy. I consider this as an approval/precedence which justifies usage of PPO in our loop.   

% \paragraph{Augmenting model-free reinforcement learning using a model.} In \cite{imagination_metacontrol,imagination_model_based_planning} a model of the environment called {\em imagination} is used to augment performance of a model-free reinforcement learning algorithm. This proved to be particularly useful in games like Sokoban, where certain moves are irreversible. 
%%SL.12.27: For this kind of thing, it would be a good idea at the end of each section to discuss how this work relates to the current one. But also this paragraph can probably be cut (you'll be out of space)
%%HM 6.01 The reason these paper are cited here is that they are about video games and at the same time they use some ideas from model-based RL.

% \paragraph{Neural architectures suitable for modeling of video games. } In this work we apply two advanced recurrent models: the Stochastic Variational Video Prediction (SV2P, \cite{sv2p}) and a video discrete autoencoder inspired by \cite{neural_discrete, auto_discrete}. 
% PM.01.08 possibly add  \cite{Buesingatal2018}


%\paragraph{Use of autoencoders.} We want a nice compact representation and run our reinforcement learning algorithm on the representation. \todo[inline]{This appears in quite a few places including \cite{raw_visual,world_models,deep_spatial,embed_to_control} but also some of pixel series \cite{pixel1,pixel2,pixel3}}

%\paragraph{Encouraging exploration.} Certainly this idea appers in \cite{video_prediction}. See also \href{http://rll.berkeley.edu/deeprlcourse/f17docs/advanced_model_learning.pdf#29}{Notes from the Berkeley course, page 29.}




% \todo[inline]{Include discussion of 3 papers mentioned in notes.}

%\todo[inline]{It would be good to find a source which really measures sample efficiency.}

%\paragraph{Worth of including here.} Schmidhuber-Huber \cite{huber} Bellemare, PhD thesis \cite{marc_skip,marc_bayesian_learning}; these all appears in related work in \cite{video_prediction}.

==> SimPLe_ICRL_submission/related_work_old_v2.tex <==
\section{Related work}
\label{sec:related_work}

% HM.1.9. a version of old related work section is in the file related_work_old.tex.
% It includes all comments, but sadly I have mingled/misplaced them in the process of re-writing.
% I am maintaining the distinction "video games vs robotics", but if necessary I am ready to drop it

%%SL.1.15: Here is a rephrasing that maintains the spirit of the original but somewhat emphasizes the distinction: Atari games gained prominence as a popular benchmark for reinforcement learning algorithms with the introduction of the Arcade Learning Environment (ALE)~\cite{}. The combination of reinforcement learning and deep models then enabled RL algorithms to learn to play Atari games directly from images of the game screen, using the DQN algorithm~\cite{dqn}, policy gradients~\cite{}, and actor-critic algorithms~\cite{}. The most successful methods in this domain remain model-free algorithms~\cite{rainbow?}. However, although the sample complexity of these methods has improved substantially over the last few years, it remains far higher than the amount of experience required for human players to learn each game~\cite{}. In this work, we aim to learn Atari games with a budget of just 100K frames, corresponding to one hour of play time. Prior methods are generally not evaluated in this regime, and we therefore reoptimized two prior methods: PPO~\cite{ppo} and Rainbow~\cite{rainbow} for optimal performance on 100K and 1M frames for comparison.
In a number of Atari games, impressive results have been achieved by the DQN algorithm \cite{dqn}. The algorithm was extended in \cite{ppo,acktr,dqn2,rainbow,a3c} towards higher performance and better parallelization.
In this work we are addressing a question what kind of performance in Atari games can be achieved within the budget of 100K frames. None of the above methods was tested against such a strict sample efficiency requirement, hence in this work we include a thorough evaluation of the PPO \cite{ppo} and Rainbow \cite{rainbow} algorithms optimized for performance on 100K and 1M frames, see Table \ref{table:rainbow}.\todo[inline]{HM @ Blazej: let us not forget about the table}

%%SL.1.15: Maybe we transition by saying: While to our knowledge no prior work has successfully learned to play a variety of Atari games with model-based reinforcement learning methods directly, multiple prior works have studied the problem of modeling Atari games, both as static videos and with action-conditioned models...
In \cite{video_prediction, recurrent} it is shown that learning of Atari 2600 environments is possible using appropriately chosen deep learning architectures. Impressively, in some cases the predictions maintain high $L_2$ accuracy over timespans of hundreds of steps. 
As learned simulators of Atari environments are core ingredients of our approach, in many aspects our work is motivated by \cite{video_prediction, recurrent}, however we focus on using video prediction in the context of learning how to play the game well and positively verify that learned simulators can be used to train a policy useful in original environments. In other terms we are making a step from a pure video-prediction task in \cite{video_prediction, recurrent} to model-based learning for Atari games.
%%SL.1.15: can probably cut this last sentence
An important step in this direction was made in \cite{video_reward_prediction}, which extends \cite{video_prediction} by including reward prediction, but does not use the model to learn policies that play the games.
Perhaps surprisingly, there is virtually no work on model-based RL in video games.
%%SL.1.15: should we say "from images"?
A notable exceptions are 
\cite{vpn,world_models}. In \cite{vpn} a model of rewards is used to augment model-free learning with good results on a number of Atari games, but the RL algorithm is not intended to be sample efficient.
%%SL.1.15: maybe instead of "but the ..." say "However, this method does not actually aim to model or predict future frames, and achieves clear but relatively modest gains in efficiency."
In \cite{world_models} a variational autoencoder is composed with a recurrent neural network into an architecture  
which is successfully evaluated in the VizDoom environment and on a 2D racing game. 
The training procedure is similar to  Algorithm \ref{alg:basic_loop}, but only one step of the loop is needed as the environments are simple enough to be fully explored with random exploration.
%%SL.1.15: I don't suppose there is anything we can include in our experiments that we can honestly say is a *comparison* to this method?

%%SL.1.15: Maybe a transition could go like this: Outside of games, model-based reinforcement learning has been explored at length for applications such as robotics~\cite{}. Though most such prior methods did not employ image observations, several recent works have sought to incorporate images into simulated~\cite{} and real-world~\cite{} robotic control.
For a survey of model-based methods for robotics see Chapter 3 in \cite{deisenroth}.
Our models of Atari environments described in Section \ref{sec:architectures} are motivated by video models developed for robotics applications in \cite{embed_to_control, deep_spatial, finn2016, sv2p, ebert, hafner, piergiovanni, paxton, rybkin-pertsch}.  Another source of an inspiration are discrete autoencoders proposed in \cite{neural_discrete, auto_discrete}.
%%SL.1.15: For this last sentence, I feel like we should instead have a separate place where we discuss related work on modeling (i.e., related prediction models)

%%SL.1.15: I think this paragraph can be merged into the discussion of model-based RL in robotics in the paragraph above. But if we want a paragraph on model-based RL methods that combine model-free optimizers and models, we can say something like this: The structure of the model-based RL algorithm that we employ consists of alternating between learning a model, and then using this model to optimize a policy by using model-free reinforcement learning within the model. Variants of this basic structure has been proposed in a number of prior works, ranging from Dyna~\cite{sutton_dyna_paper} to more recent methods that incorporate deep networks for models and policies... [and can cite/discuss here the ensemble paper (i.e., the discussion below), as well as stochastic value gradients, model-based value expansion, and this paper: Kalweit, Gabriel and Boedecker, Joschka. Uncertainty driven imagination for continuous deep reinforcement learning]
In a recent work \cite{trpo_ensemble} a training loop similar to one described in  Algorithm \ref{basic_loop} along with a policy gradient algorithm \cite{trpo} were applied to a number of robotic tasks in the MuJoCo physics simulator \cite{mujoco}.  This successful application of a learned model and a policy gradient algorithm motivated our choice of PPO \cite{ppo} as the algorithm which improves policy in the learned environment, see also discussion in Section 3.3.2.1 of \cite{deisenroth}. % "To the best our knowledge  knowledge, there are currently not many approaches for model-based policy  search  based  on  sampling-based  gradients  using  the  methods from Section 2."

% Two student papers on MBRL for Atari (Pong, specifically)
% http://cs231n.stanford.edu/reports/2016/pdfs/116_Report.pdf
% https://dspace.fandm.edu/bitstream/handle/11016/24289/Foley_Thesis.pdf?sequence=1&isAllowed=y
%%CF: I don't think we need to worry about citing these.

==> SimPLe_ICRL_submission/rl_algorithm.tex <==
\section{Reinforcement learning algorithm}
\label{sec:rl}

\textbf{pm: under construction do not change}

Given a stochastic policy $\pi$, which for a given state assigns probability distribution over possible actions, we define the value function $V_\pi(s) := \mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s=s_0 \right)$. We define $\eta(\pi)$ to be the value function, when the initial state is sampled according to $\rho_0$. The goal of reinforcement learning is to find a policy which maximizes $\eta$.

In our experiments the reinforcement learning part of the loop in Figure \ref{figure_basic_loop} (Algorithm \ref{basic_loop}, line 6) is performed with the Proximal Policy Optimization algorithm (PPO, \cite{ppo}). PPO is a general purpose model-free reinforcement learning algorithm. This kind of algorithm can be considered as a black-box in this project. The black-box works for a prescribed number of epochs. In a single epoch it gathers new episodes and using experience from the episodes it improves the policy. % The procedure is motivated by the DAgger algorithm \cite{dagger} and presented below in Algorithm \ref{basic_loop}.

\paragraph{Training of a reinforcement learning agent}
% TODO: details about PPO, update figure below.
% latex source https://www.overleaf.com/16266511yhyscgmyhztg
% \begin{figure}[H]
% \centering
% \includegraphics[width=4in]{figures/network_ppo.png}
%  \end{figure}

==> SimPLe_ICRL_submission/tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput


==> SimPLe_ICRL_submission/tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput


==> analysis_old.tex <==
\section{Analysis}

To be included in this section
\begin{enumerate}
    \item ablation: number of training loops
    \item (?) ablation: PPO training on real env
    \item model measures (next frame accuracy, long term value prediction) don't determine final RL performance - how well we can justify it?
    \item  shared weights WM/P models
    \item effects of limited horizon -- e.g. pong/pacman doesn't restart, montezuma dies when jumping in place;
    bank heist story why stochastic model is better - not true?
    \item using of random starts is essential (?)
\end{enumerate}

\todo[inline]{All text in this section is just a placeholder; for mode details see the doc}
\label{envs}
\label{sec:envs}
% \todo[inline]{Here we describe interesting environments; this was quite nicely done in Chiappa's work as well as in Oh's work and this is the place where we want to discuss BankHeist}
In this section we describe \pong, \breakout\ and \freeway\ environments. These environments were introduced in the Arcade Learning Environment (ALE) \cite{ale} (see also \cite{ale2} for a current overview of challenges and successes of various learning methods in ALE). 

\paragraph{Dimensions of input and output.} The screen as given by the ALE emulator consists of an RGB image of the size $160\times 210$ pixels\todo[inline]{Is it rally true?}.  The action space consists of up to 18 actions\todo[inline]{MB.1.16: this is game dependent}. The reward in all games is an integer number\todo[inline]{MB.1.16: which we truncate to -1 0 and 1}.

\paragraph{\pong.} In \pong\ the player is expected to move the green paddle. The red paddle is operated by the original game AI. If the ball crosses the left end of the screen, then the green player scores a point. If the ball crosses the right end of the screen, then the red player scores a point. The total reward for the game is the difference between points scored by the green player and the red player. A full episode lasts until one of the agents scores 21 points. An environment for \pong\ was trained in \cite{recurrent}. Authors reported occasional disappearance of the ball and blurriness of paddles. In order to simplify learning of the environment we considered a modified environment with a ball of the size $10\times 10$ pixels. The change concerns only the observation and not rules of the game. 

\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__3.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__9.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/PongDeterministic-v4__31.jpg}%
}%
\caption{Four frames from the \pong\ environment. }
\label{fig:pong_original}
\end{figure}


\paragraph{\breakout.} In \breakout\ the player is expected to move the paddle located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model, see page 18 of \cite{recurrent}. As in the case of \pong\ in the modified environment we allowed for a ball of the size $10\times 10$ pixels.

% \begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__2.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__3.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/BreakoutDeterministic-v4__6.jpg}%
}%
\caption{Four frames from the original \breakout\ environment. }
\label{fig:breakout_original}
\end{figure}
% \end{comment}

\begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__1.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__2.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures_mod/BreakoutDeterministic-v4__4.jpg}%
}%
\caption{Four frames from the modified \breakout\ environment. }
\label{fig:breakout_mod}
\end{figure}
\end{comment}

\paragraph{\freeway.} In \freeway\ the player is expected to move the yellow chicken from the bottom of the screen to the top of the screen.  The chicken moves only vertically. A point is obtained in the game if the chicken reaches the top of the screen. There is no concept of life, but if the chicken is hit by a car, then it falls approximately 2 lanes down. The environment makes appearance in \cite{recurrent} and is considered as an easy environment to model \cite[page 18]{recurrent} frames. The problem though are the sparse rewards, since the only time a non-0 reward occurs is at the top of the screen.  

%\begin{comment}
\begin{figure}[H]
\makebox[\columnwidth]{%
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__4.jpg}%
\hfill
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__6.jpg}%
\hfill    
\includegraphics[width=0.24\columnwidth]{figures/FreewayDeterministic-v4__8.jpg}%
}%
\caption{Four frames from the original \freeway\ environment. }
\label{fig:breakout_mode}
\end{figure}
% \end{comment}

\paragraph{\bankh.} \todo[inline]{Here Łukasz includes his take on \bankh}


\paragraph{Improvements to performance over iterations}

We trained the iterative algorithm for 3 epochs of
the world-model/ppo/generate-data loop. In Figure~\ref{fig:freeway_three_epochs} we present
how the results change on the example of \freeway. Note that in the first step the environment is not producing rewards
correctly. It only learns to produce them in the second step and the results get high in the third. See the caption of the Figure and
\href{https://sites.google.com/view/modelbasedrlatari/home}{webpage}\footnote{\url{https://sites.google.com/view/modelbasedrlatari/home}} for 
videos showing progress of the agent. %[TODO: show chicken from the video unsure near the top?]

\begin{figure}[H]
\centering
\includegraphics[width=0.9\columnwidth]{figures/freeway.png}
%\includegraphics[width=1.8in]{figures/c0.png}
%\includegraphics[width=1.8in]{figures/c1.png}
%\includegraphics[width=1.8in]{figures/c3.png}
\caption{Three different runs of PPO training on simulated environment $env'$ for three iterations of the whole loop on \freeway\ training.
  The first iteration is epochs 0-50, the next 50-100 and the final one 100-150. Note that while all 3 models only reach scores below 4 in
  the shortened PPO training, all of them actually get scores above 10 when playing in the real environment, and the two better runs get above 20.
  Two of the runs already reach positive scores in the first iteration, while one run (orange) only reaches them in the second iteration -- this
  happens because no reward was seen in the first randomly generated data. In the third iteration the policies of the two runs that saw rewards
  in the first iteration get very good (scores above 20), while the third one learns slower.}
\label{fig:freeway_three_epochs}
\end{figure}

\paragraph{The accuracy metric on selected games.}\todo[inline]{(Henryk) @Piotr, I am assuming that you will fix it or remove}

\paragraph{Metrics}
We propose a new \textit{correct rewards predictions per sequence} metric to evaluate simulated environments. 
Let $t = (s, acs)$ be a tuple consisting of a state $s$ and a sequences of actions $acs$. We say that $env'$ is successful on $t$ if started from $s$ it produces the same total reward as the $env$ while executing subsequently actions $acs$.
Given $D$, a set of tuples as above we define \textit{correct rewards predictions per sequence} ratio on $D$ to be the ratio of successful $t$'s in $D$.
Typically, we evaluate simulated environment on $D$ with sequences $acs$ of a prescribed length $n\in \mathbb{N}$ generated according to some stochastically perturbed policy $\pi$. Intuitively, having good ratio in such a test means that the model behaves reliably in the neighborhood of $\pi$ in the time horizon $n$. %\todo{Piotr have a look here} %Thus, hopefully, it can be used in a reinforcement learning algorithm. 
We argue that this metric can correctly measure resemblance  of the simulated and original dynamics.  We believe it is better than the standard $L_2$ accuracy used in \cite{video_prediction,recurrent}, which has tendency to omit small but important objects (e.g. the ball in \pong).
\todo[inline]{So far we have one case: Pong, and number are very old, see Figure \ref{fig:correctness}}

\begin{figure}[H]
\includegraphics[width=0.35\textwidth]{figures/pong_ratio}%

\caption{Results on \pong: metric of correctness of rewards predictions per sequence.}
\label{fig:correctness}
\end{figure}

\paragraph{Analysis of the PPO modification}
\todo[inline]{So far we have one case: Pong, and number are very old, see Figure \ref{fig:ppo_mod}}

\begin{figure}[H]
\includegraphics[width=0.35\textwidth]{figures/compare1000steps}
\caption{Results on \pong: a comparison of training in two settings: one assuming 0 reward at the end of simulated environment episode and improved version using value function estimation instead.}
\label{fig:ppo_mod}
\end{figure}

==> architectures_old.tex <==
\section{World models}
\label{sec:architectures}
\label{sec:training}

%%SL.12.27: Perhaps organizationally it would be better to first have a top-level Overview section to describe the parts of the method, and then a single top-level section with the name of the method, with subsections about the individual parts of the method? If the goal of this section is to discuss predictive model architectures, perhaps that would also make for a better section title: Predictive Model Architectures or something? The title of the first paragraph "Architecture of a Neural Simulator" could also work well (note however that in the deep learning community, "neural simulator" sometimes takes on a very specific meaning as an object-decomposed model that emulates the high-level design of a physics simulator)

% Dumitru. here is how I would structure this: 1-2 sentences about what we are looking for in a world model (stochasticity, scalability, stability). Say that to this end we came up with a new architecture that is straightforward but that is novel for video prediction. Also say that we compare with SV2P, and describe it. Then go into the details of the filter sizes and training losses: first the stuff that is common to both, then the specifics for each model. Alternative proposal is to describe the details of the world model training that are common first, and then describe the models themselves.}

%%SL.12.27: It could be a good idea at the beginning of this paragraph to explain the problems that the architecture design is trying to address so as to motivate the design decisions.
\paragraph{Architecture of a neural simulator of an environment. } Our basic architecture, presented in Figure~\ref{fig:kanapa}, resembles the convolutional feedforward network from \cite{video_prediction}.  The input $X$ consists of a few consecutive game frames and an action $a$. The visual input is processed by stacked convolution layers. The actions are one-hot-encoded and embedded in a vector which is multiplied channel-wise with the output of the conv layers. It is then processed by fully connected layers and deconvolved. The network outputs the next frame of the game and the value of reward.% Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

	In most of our experiments we choose the input to be four frames as with our choice of environments they fully identify the state of the game. The network is the workhorse of our simulated environment $env'$. The environment contains a memory $M$ of four frames, which is initialized with frames retrieved for the original environment. Given an action $a$ the tuple $(M,a)$ is processed by the network outputting a new frame and a reward $r$. The oldest frame of $M$ is discarded and the new one is included. 

%\todo{pm: The next section is too much of storytelling}
%\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games.
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design the same is true about the ouput $X'$.
%\todo{Important: no pooling}

In our experiments we varied details of the architecture above. In most cases we use a stack of four conv layers with $64$ filters followed by three dense layers (the first two have $1024$ neurons). The dense layers are concatenated with $64$ dimensional vector with a learnable action embedding. Next, three deconv layers of $64$ filters follow. An additional, final, deconv layer outputs an image of the original $210\times 160$ size. The number of filters is either $3$ or $2\times 256$. In the first case the output is a real-valued approximation of pixel's RGB value. In the second case filters are followed by softmax producing probability distribution on the color space. The reward is predicted by a softmax attached to the last fully connected layer. 
We used dropout equal to $0.2$ and the layer normalization. 

We have also experimented with Stochastic Variation Video Prediction (SV2P)~\cite{sv2p}, a recent technique that incorporates a latent variable model with a generative recurrent network. The latter is a convolutional LSTM from \cite{cdna} that internally predicts transformations of the context images conditioned on latent values, actions and the previous frames. The model is trained with the reparametrization trick and allows for efficient inference at test time. When successfully trained, it make it possible to sample diverse and plausible action-conditioned futures. For the Atari experiments, we followed the same protocol of training as with the basic convolutional model described above. Note that generally speaking the multiplier for the KL-loss $\beta$ has to be tuned on a per-game basis: we tried 3 such values per game (TODO: confirm with mbz how many we actually tried).\todo[inline]{The reference to KL-loss may require some elaboration or abstraction.}

% MB.1.17 commenting this out
% \begin{figure}[H]
% \centering
% \includegraphics[width=3.5in]{figures/sv2p}
% \caption{The Stochastic Variational Video Prediction model (SV2P) by \cite{sv2p}}
% \label{fig:sv2p}
% \end{figure} 

\paragraph{Loss functions}
The visual output of our networks are either one float per pixel/channel or the categorical 256-dimensional softmax. 
In the case of the real output we used the \textit{clipped $L_2$ loss}, viz. $\max(x^2 - C, 0), C>0$. We found that clipping was crucial for improving prediction power of the models (both measured with the correct rewards predictions per sequence metric and successful trainings using Algorithm \ref{dpll}). We conjecture that the clipping substantially decreases the magnitude of gradients stemming from fine-tuning of big areas of background consequently letting the optimization process to concentrate on small but important areas (e.g. the ball in Pong). Setting $C$ corresponding to $10$ pixels worked particularly well in our experiments. 
We used similar trick for the softmax outputs, namely we clipped the cross-entropy loss once the model achieved high level of confidence about a pixel value (we used $98\%$ in our experiments). As in the first case, clipping was crucial for obtaining well performing models. 

\paragraph{Scheduled sampling}
By design, the clipped loss does not produce accurate pictures. The simulator $env'$ consumes its own predictions from previous steps thus, due to compounding errors, the model may drift out of the area of its applicability. We mitigate this problem by randomly replacing in training some frames of the input $X$ by one step predictions. Typically, we increase the mixing probability during training arriving to $50\%$. 

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_det.pdf}
\caption{Architecture of deterministic model which consists of a skip-connected convolutional encoder and decoder. The input to the model is four stacked frames as well as the selected action while the output is the next predicted frame and expected reward. Input pixels and action are embedded using fully connected layers and there is per-pixel softmax ($256$ colors) in the output.}
\label{fig:model_det}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_stoch.pdf}
\caption{Architecture of stochastic model. The generative network is the same as Figure~\ref{fig:model_det} with an additional convolutional inference network to approximates the posterior given the next frame. The latent values will be sampled from approximated posterior and an assumed prior of $\mathcal{N}(\mathbf{0}, \mathbf{I})$ at training and inference time respectively.}
\label{fig:model_stoch}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.8\textwidth]{figures/model_basic_disc.pdf}
\caption{Architecture of stochastic model with discrete latent. The overall architecture of this models is similar to Figure~\ref{fig:model_stoch} with two main differences. First, at training time, the sampled latent values from the approximated posterior will be discretized into bits. The backpropagation bypasses the discretization similar to~\citet{van2017neural}. A third LSTM based network is trained to approximate each bit given the previous ones. At inference network, the latent bits are predicted auto-regressively using this network.} 
\label{fig:full_discrete}
\end{figure*}



% \section{Design and training of simulators}
% \label{sec:architectures}

% \paragraph{Architecture of a neural simulator of an environment. } Our basic architecture, see Figure \ref{fig:kanapa}, resembles the convolutional {\em feedforward} architecture from \cite{video_prediction}.  The input $X$ consists of $4$ game frames and the action $a$. The visual input is processed by stacked convolution layers. The actions are one-hot-encoded and then embedded in a vector which is concatenated with the the output of the conv layers. It is then processed by some fully connected layers and deconvolved. The output of the network is the next gameframe and the value of reward. Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

% %\todo{pm: The next section is too much of storytelling}
% %\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games. 
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design the same is true about the ouput $X'$. 
% %\todo{Important: no pooling}

% In our experiments we varied a number of layers, but the most standard architecture of the encoder consists of $4$ convolutional layers with 128 filters, followed by 3 dense layers. The third of the layers marked as $e$ in Figure \ref{fig:kanapa} is stacked with the embedding of actions marked as $a$ in Figure \ref{fig:kanapa}. The stacked layer is followed by $4$ deconvolutions.     

% \paragraph{Metrics}
% In our work we mostly abandonded $L_2$ metric as a measure of accurracy. We argue that in many cases it is not well suited to asses the models as it underweights meaning small (but potentially crucial) objects. Instead we introduce \textit{correct rewards per sequence} parametrized by the sequence length $n$. By definition the metric is the ratio of action sequences in the training/eval set for with $env'$ predicts total reward consistent with the one of $env$.

% \paragraph{Loss functions}
% Our experiments followed two lines. The first output was a single real value for each pixel and channel, in the second we used categorical output of 256-dimensional softmax. 

% For both losses we introduced a clipping factor: the final loss was $\max(loss - C, 0)$ for a constant $C>0$. We found that clipping was crucial for improving prediction power both over the standard $L_2$ loss and over the standard cross-entropy loss. We conjecture fine-tuneing of big areas of background the clipping substantially decreases the magnitued of gradients stemming from fine-tuneing of big areas of background consequnetly letting the optimisation process to concentrate on small but important areas, like the ball in Pong. We used $C = 0.01$ for cross-entropy loss (so the model did not get any benefit from being more than 99\% confident about any pixel value) and $C = 10$ for $L_2$ loss so
% that being within $3$ RGB values was considered sufficient.

% \paragraph{Mixing.} \todo{Add mixing}

% \paragraph{Resets.} \todo{Add resets}



%\cite{video_prediction,recurrent}. 
%Important points: the encoder-decoder architecture, prediction-dependent transition, observation-dependent transition, long-short term accuracy. 

%\paragraph{Training of a simulator of an environment}
%Some decisions.
%\todo[inline]{which models we want to discuss? Loss functions, layer details, mixing, metrics such as percent of successful trajectory-reward predictions, {\bf negative mining} (Henryk) Yes, we want to discuss, details of training to be described by Piotr}

%\input{figures/kanapa_network.tex}
% source: https://raw.githubusercontent.com/PetarV-/TikZ/master/Convolutional%20autoencoder/convolutional_autoencoder.tex
% overleaf copy (can be modified): https://www.overleaf.com/16266360vmyxnwdwdnpn

%Do we want a figure like\todo{The figure is missing actions and rewards, but this can be fixed}
% \begin{figure}[H]
% \centering
% \includegraphics[width=5.5in]{figures/new_arch.png}
% \caption{A simplified view of our encoder-decoder architecture.}
% \label{fig:kanapa}
% \end{figure}



==> big_unfinished_table.tex <==
% \paragraph{Big table}
% \setlength{\belowcaptionskip}{-17pt}
%\begin{wraptable}{r}{0.55\textwidth}
\begin{table}[H]
%\vspace{-17pt}
\begin{center}
{\scriptsize{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
Game          & random & ours@200K & ours@200(*) & ours@1M  & PPO@200K & PPO@1M & PPO@10M &  Dop \\
\hline
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Pong           & -20.335 & 20         & 20.7    \\
Breakout       & 1.105   & 8          & 274.8     \\
Freeway        & 0.005   & 26         & 32.5    \\
Boxing         & 1.04    & 32         & 94.6     \\
Crazy Climber  & 7565    & 35800      & 110202 \\
Kung-Fu Master & 594     & 2600       & 23310.3  \\
Frostbite      & 73.6    & 260        & 314.2   \\
Seaquest       & 79.2    & 260        & 1204   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
Hero           & 378.9   & 2990       & not reported  \\
Berzerk        & 146.55  & 920        & not reported   \\
\hline
\end{tabular}
}}}
\end{center}
\label{tab:main}
\caption{Our model-based results for 42 games trained using various algorithms: 100K ours at 200K and 1M, ours@200(*)  - an impure version of our algorithm which is allowed to train on a real environment, PPO and Dopamina.}  
\end{table}

==> conclusion_old.tex <==
\section{Conclusions and future work}

%%SL.1.22: Here is a suggested rephrasing of the paragraphs below (similar content, just organized a bit differently):
% We presented a model-based reinforcement learning approach that can operate directly on raw pixel observations, and can learn effective policies to play games in the Atari Learning Environment. Our experiments demonstrate that our approach can learn to play many of the games with just $100$K transitions, corresponding to ??? hours of play time. In many cases, the number of samples required for prior methods to learn to reach the same reward value is several times larger.
%
% While the predictive model in our experiments has stochastic latent variables, the Atari games that we evaluate on are largely deterministic. Studying stochastic domains is an exciting direction for future, and we expect that effective probabilistic modeling of dynamics would be effective in such settings also. Another interesting direction for future work is to study other ways in which the predictive neural network model could be used. Our approach utilizes the model as a learned simulator, and then directly uses model-free policy search methods to acquire the behavior policy. However, since neural network models are differentiable, the additional information contained in the dynamics gradients could itself be incorporated into the reinforcement learning process. Finally, the representation learned by the predictive model is likely to itself be more meaningful than the raw pixel observations from the environment, and incorporating this representation into the policy could further accelerate and improve the reinforcement learning process.
%
% As a long-term challenge, we believe that model-based reinforcement learning based on stochastic predictive models represents a promising and highly efficient alternative to model-free RL, and applications of such approaches to both high-fidelity simulated environments and real-world data represent an exciting direction for future work that can enable highly efficient learning of behaviors from raw sensory inputs, in domains such as robotics and autonomous driving.

%%SL.1.22: Some general rationale: let's try to keep prior work to the prior work section, it often comes across as pretty unsatisfying to have a discussion section that says something like "prior word did this, maybe we can do it too in future work" (if it was done in prior work, then it's not future work). It's also important to leave the reader with a very positive impression of the work, so while discussing some limitations is really important, it's also a good idea to use these to frame exciting future work that goes beyond the current method.

We presented a number of ideas that, taken together, allow to train Atari games end-to-end in a model-based way and get improvements in data efficiency.
While in this work we focus on deterministic environments, it would be interesting to study stochastic environments, possibly exploiting methods from \cite{world_models}. This would open possibly of using model-based reinforcement learning techniques in real-world unstructured scenarios, for example competing in a video game against human players. 

In some of our experiments we output probability distributions over pixel values. We conjecture that their entropy/variance can serve a measure how model is confident about its own predictions. We mention \cite{trpo_ensemble} which introduced model ensembles with a similar purpose. Measuring confidence is a challenging task with multiple possible applications. On the one hand, it might be used to determine trust regions for policy optimization, resulting in a more stable execution of Algorithm~\ref{alg:basic_loop}. On the other hand, creating an incentive to enter low confidence regions might be a useful exploration strategy. 

Finally, there are many benefits of having a neural net model of a game. Its hidden state is smaller and possibly more semantically meaningful than visual input and could be used as an input for policy. As called for in \cite{modelplanning}, one could use it for model-based planning and propagate gradients though the model. Finally, there are many technical benefits as the neural network model runs on the same accelerator that trains the policy and can be ran in batch mode, greatly simplifying the architecture of the RL setup and speeding up computations for more complex environments.

As a long-term challenge, we would like to deal with visually rich simulated robotics environments such like Carla \cite{carla}. Compressing states as shown in \cite{world_models} is particularly appealing as such approach could be used in mixed scenario where the compression is learn using simulated data and later used for rapid reinforcement learning on real-world data. 

==> environments.tex <==
\section{Atari environments}
\label{envs}
\label{sec:envs}
% \todo[inline]{Here we describe interesting environments; this was quite nicely done in Chiappa's work as well as in Oh's work and this is the place where we want to discuss BankHeist}
In this section we describe \pong, \breakout\ and \freeway\ environments. These environments were introduced in the Arcade Learning Environment (ALE) \cite{ale} (see also \cite{ale2} for a current overview of challenges and successes of various learning methods in ALE). 

\paragraph{Dimensions of input and output.} The screen as given by the ALE emulator consists of an RGB image of the size $160\times 210$ pixels\todo[inline]{Is it rally true?}.  The action space consists of up to 18 actions. The reward in all games is an integer number.

\paragraph{\pong.} In \pong\ the player is expected to move the green paddle. The red paddle is operated by the original game AI. If the ball crosses the left end of the screen, then the green player scores a point. If the ball crosses the right end of the screen, then the red player scores a point. The total reward for the game is the difference between points scored by the green player and the red player. A full episode lasts until one of the agents scores 21 points. An environment for \pong\ was trained in \cite{recurrent}. Authors reported occasional disappearance of the ball and blurriness of paddles. In order to simplify learning of the environment we considered a modified environment with a ball of the size $10\times 10$ pixels. The change concerns only the observation and not rules of the game. 

\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__3.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__9.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/PongDeterministic-v4__31.jpg}%
}%
\caption{Four frames from the \pong\ environment. }
\label{fig:pong_original}
\end{figure}


\paragraph{\breakout.} In \breakout\ the player is expected to move the paddle located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model \cite[page 18]{recurrent}. As in the case of \pong\ in the modified environment we allowed for a ball of the size $10\times 10$ pixels.

%\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__2.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__3.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/BreakoutDeterministic-v4__6.jpg}%
}%
\caption{Four frames from the original \breakout\ environment. }
\label{fig:breakout_original}
\end{figure}
%\end{comment}

\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__1.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__2.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures_mod/BreakoutDeterministic-v4__4.jpg}%
}%
\caption{Four frames from the modified \breakout\ environment. }
\label{fig:breakout_mod}
\end{figure}
\end{comment}

\paragraph{\freeway.} In \freeway\ the player is expected to move the yellow chicken from the bottom of the screen to the top of the screen.  The chicken moves only vertically. A point is obtained in the game if the chicken reaches the top of the screen. There is no concept of life, but if the chicken is hit by a car, then it falls approximately 2 lanes down. The environment makes appearance in \cite{recurrent} and is considered as an easy environment to model \cite[page 18]{recurrent} frames. The problem though are the sparse rewards, since the only time a non-0 reward occurs is at the top of the screen.   % located at the bottom of the screen. The paddle can be moved in the and right directions to the end of the screen. When the ball hits the wall of the bricks, points are scored depending on the color of the brick. The player has 5 lives and the beginning of the game. A life is lost whenever the ball crosses the bottom of the screen.  The environment makes appearance in \cite{recurrent} and is considered as a difficult environment to model \cite[page 18]{recurrent}.  

%\begin{comment}
\begin{figure}[H]
\makebox[\textwidth]{%
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__0}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__4.jpg}%
\hfill
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__6.jpg}%
\hfill    
\includegraphics[width=0.24\textwidth]{figures/FreewayDeterministic-v4__8.jpg}%
}%
\caption{Four frames from the original \freeway\ environment. }
\label{fig:breakout_mode}
\end{figure}
% \end{comment}

\paragraph{\bankh.} \todo[inline]{Here Łukasz includes his take on \bankh}


==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}

We evaluate SimPLe on a suite of Atari games from Atari Learning Environment (ALE) benchmark.
In our experiments, the training loop is repeated for 15 iterations, with $6400$ interactions with the environment collected in each iteration.
We apply a standard pre-processing for Atari games: a frame skip equal to 4, that is every action
is repeated 4 times and frames are down-scaled by a factor of 2.

Because some data is collected before the first iteration of the loop,
altogether $6400 \cdot 16 = 102,400$ interactions with the Atari environment are used during training.
This is equivalent to $409,600$ frames from the Atari game (114 minutes in NTCS, 60 FPS).
All our code is available. \textbf{TODO: more?}
% as part of the Tensor2Tensor library with instructions on how to run our experiments.\footnote{\url{https://github.com/tensorflow/tensor2tensor/tree/master/tensor2tensor/rl}} 

At every iteration, the latest policy trained under the learned model is used to collect data in the real environment $\env$.
Due to vast difference between number of training data from simulated environment and real environment (15M vs 100K) the impact of real data on policy is negligible.

 We evaluate our method on $26$ games selected on the basis of being solvable with existing state-of-the-art model-free deep RL algorithms\footnote{Specifically, for the final evaluation we selected games which achieved non-random results using our method or the Rainbow algorithm using $100$K interactions.}, which in our comparisons are Rainbow~\citep{rainbow} and PPO~\citep{ppo}.
 For Rainbow, we used the implementation from the Dopamine package and spent considerable time tuning it for sample efficiency.

For visualization of all experiments see \url{https://goo.gl/itykP8}
and for a summary see Figures \ref{fig:compare_dopamine} and  \ref{fig:compare_ppo}.
It can be seen that our method is more sample-efficient than a highly tuned Rainbow baseline on almost all games, requires less than half of the samples on more than half of the games and, on \freeway\, is more than 10x more sample-efficient. Our method outperforms PPO by an even larger margin.


==> figures/kanapa_network.tex <==
\begin{figure}
\begin{tikzpicture}[scale=0.1,every node/.style={scale=0.1}]]

	\node (1) [draw, dashed, minimum height=15em, minimum width=62em, xshift=24em, fill=olivegreen, fill opacity=0.2, very thick, rectangle, rounded corners] {};
		\node (la1) [below=0em of 1] {{\emph{encoder}}};
	\node (2) [draw, dashed, minimum height=14em, fill = red, fill opacity=0.2,minimum width=35em, xshift=63.5em, very thick, rectangle, rounded corners] {};
		\node (la1) [below=0em of 2] {{\emph{decoder}}};

	\node[] (i2) {};
	\pic[fill=green!50] (I2) {cube={1.8/1.8/0.4/1}};
	
	\togglefalse{redraw}
	\togglefalse{redraw2}
	
  	\node[right=16em of i2] (y) {};
  	
  	\pic[right=16em of i2, fill=echoreg!50] (Y) {cube={1.8/1.8/1/1}};
  	
  	\node[right=12em of y] (y1) {};
  	\pic[right=12em of y, fill=red!50] (Y1) {cube={0.9/0.9/1/1}};
  	
  	\node[right=12em of y1] (y2) {};
  	\pic[right=12em of y1, fill=echoreg!50] (Y2) {cube={0.9/0.9/2/1}};
  	\node[right=10em of y2] (y3) {};
  	\pic[right=10em of y2, fill=red!50] (Y3) {cube={0.45/0.45/2/1}};
  	
  	\node[right=9em of y3] (z1) {};
  	\pic[right=9em of y3, fill=mymauve!50] (Z1) {cube={0.9/0.9/1/1}};
  	
  	\node[right=12em of z1] (z2) {};
  	\pic[right=12em of z1, fill=mymauve!50] (Z2) {cube={1.8/1.8/0.4/1}};
  	
  	\draw [-stealth, ultra thick] (I2-B) -- node[above] {Conv.} node[below] {ReLU} (Y-A);
  	
  	\draw [-stealth, ultra thick] (Y-B) -- node[above] {Pool} (Y1-A);
  	
  	\draw [-stealth, ultra thick] (Y1-B) -- node[above=0.3em, inner sep=0.1em] {Conv.} node[below] {ReLU} (Y2-A);
  
  	\draw [-stealth, ultra thick] (Y2-B) -- node[above] {Pool} (Y3-A);
  	
  	
  	\draw [-stealth, ultra thick] (Y3-B) -- node[above] {Deconv.} node[below] {ReLU} (Z1-A);
  	
  	\draw [-stealth, ultra thick] (Z1-B) -- node[above] {Deconv.} node[below] {logistic} (Z2-A);
  	
  	
  	\color{black}
  	
  	\toggletrue{redraw}
  	\toggletrue{redraw2}
  	
  	\node[right=16em of i2] (y) {};
  	\pic[right=16em of i2, fill=echoreg!50] (Y) {cube={1.8/1.8/1/1}};
  	
  	\pic[right=12em of y, fill=red!50] (Y1) {cube={0.9/0.9/1/1}};
  	
  	\pic[right=12em of y1, fill=echoreg!50] (Y2) {cube={0.9/0.9/2/1}};
  	
  	\pic[right=9em of y3, fill=mymauve!50] (Z1) {cube={0.9/0.9/1/1}};
  	
  	\togglefalse{redraw2}
  	
  	\pic[right=10em of y2, fill=red!50] (Y3) {cube={0.45/0.45/2/1}};
  	
  	\toggletrue{redraw2}
  	
	\node[] (i2) {\LARGE ${\bf X}$};
  	\node[right=9.25em of y2] (y3) {\LARGE ${\bf z}$};
  	\node[right=11em of z1] (z2) {\LARGE ${\bf X}'$};

\end{tikzpicture}
\label{fig:kanapa_net}
\end{figure}

==> figures/the_loop.tex <==
\begin{figure}[H]
\centering
\begin{tikzpicture}[node distance = 0.9cm, thick, scale=1., 
every node/.style={scale=1.}, nodes = {align = center},>=latex]
  \node[Minimum Width = loop, shape = ellipse, fill = red] (imp-sol)
    {\texttt{Gather observations and rewards using $\pi$ in $\env$}\\ 
    \texttt{and use them to improve model $\env'$}};
  \node[Minimum Width = loop, fill = yellow, below = of imp-sol] (rec-box)
    {\texttt{train $\pi$ in $\env'$}\\ \texttt{using a model-free algorithm}};
  \node[shift = (left:.7*x_node_dist)] at
    ($(imp-sol.west|-imp-sol.south)!.5!(rec-box.north west)$) (for-1) {};
  \node[above = of for-1] (for-3) {};
    % {$\texttt{action}$};
  \node[shift = (right:.7*x_node_dist),minimum size = 0pt] at
    ($(imp-sol.east|-imp-sol.south)!.5!(rec-box.north east)$) (for-2) {};
  \node[above = of for-2] (for-4) {};
    % {$\texttt{state}$};
  \begin{scope}[on background layer]
    \node[fit = (for-1)(for-2)(imp-sol)(rec-box), basic box = blue,
      header = Vanilla model-based RL loop] (dmft-l) {};
  \end{scope}
  % \draw[->] (rec-box) |- ++(1,-1) |- (imp-sol);
  % \path[very thick, blue, hv] (rec-box) edge[->] (for-1) edge[<-] (imp-sol);
  \path[very thick, blue, hv] (rec-box) edge[-] (for-3) edge[<-] (for-4)
                              (imp-sol) edge[-] (for-4) edge[<-] (for-3);

%  \node[left = of dmft-l, basic box = green, header = Corpus]
%    (dmft-p) {};
%  \path[fat blue line, ->, dashed, vh] (dmft-p) edge
%    ({$(dmft-p.east)$}-|dmft-l.west);
\end{tikzpicture}
\caption{The learning model-based learning loop; $\env$ is the original game and $\env'$ is a simulator of $\env$. }
\label{figure_basic_loop}
\end{figure}

==> figures_mod/architectures.tex <==
\section{World Models}
\label{sec:world_models}
\label{sec:architectures}
\label{sec:training}

%\begin{comment}
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\textwidth]{figures/model_basic_disc.pdf}
%\includegraphics[width=1.\textwidth]{figures/cycle.pdf}
\caption{Architecture of the proposed stochastic model with discrete latent. The input to the model is four stacked frames (as well as the action selected by the agent) while the output is the next predicted frame and expected reward. Input pixels and action are embedded using fully connected layers, and there is per-pixel softmax ($256$ colors) in the output. This model has two main components. First, the bottom part of the network which consists of a skip-connected convolutional encoder and decoder. To condition the output on the actions of the agent, the output of each layer in the decoder is multiplied with the (learned) embedded action. Second part of the model is a convolutional inference network which approximates the posterior given the next frame similar to~\citet{sv2p}. At training time, the sampled latent values from the approximated posterior will be discretized into bits. To keep the model differentiable, the backpropagation bypasses the discretization following~\citet{auto_discrete}. A third LSTM based network is trained to approximate each bit given the previous ones. At inference time, the latent bits are predicted auto-regressively using this network. The deterministic model has the same architecture as this figure but without the inference network.} 
\label{fig:full_discrete}
\end{figure*}
% \end{comment}


% In principle any model that approximates the following transition function can be used as a world model:
%$$
% $(s_{t+1}, r_{t+1}) = T(s_{0:t}, a_{0:t})$
%$$
% where $s_t, a_t,$ and $r_t$ are the state, action and reward at time-step $t$. Hence, any world model has two major components: next frame predictor and reward predictor. 

%In practice, scalability and stability of a model are crucial which limits the practicality of current video prediction models. We found out that merging the reward predictor and frame predictor helps with both performance and convergence speed. More precisely, merging the reward model can help the next frame predictor to get \textit{more important} pixels right whereas in the absence of such signal the video model receives an equal penalty for each pixel.

A crucial decision in the design of world models   % introduced in Section \ref{sec:mbrl}
% Another crucial design element for designing an effective world model 
is the inclusion of stochasticity. Although Atari is known to be a deterministic environment, it is stochastic given only a limited horizon of past observed frames (in our case $4$ frames). The level of stochasticity is game dependent; however, it can be observed in many Atari games. An example of such behavior is the \textit{pause} after a player scores in \texttt{Pong}. These pauses are longer than 4 frames, so a model looking at only the past 4 frames does not know when a new round of the game should start and may keep predicting paused frames.
% \todo[inline]{BO1.21. Have we ever observed stochastic model escaping from pause state? Although it should be able to do it in theory, I haven't seen examples of this. I think that random starts are what fixes this issue.\\MB.1.22 I did observe this with SV2P.\\ LK.1.22: I did see it with SD.}

% Considering these challenges, 
In search for an effective world model we have experimented with various architectures, both new and modified versions of existing ones. In this section, we describe the architectures and the rationale behind our design decisions.  In Section \ref{sec:analysis} we compare the performance of these models.



\subsection{Deterministic Model}
Our basic architecture, presented as part of Figure~\ref{fig:full_discrete}, resembles the convolutional feedforward network from \citet{video_prediction}.  The input $X$ consists of four consecutive game frames and an action $a$. Stacked convolution layers process the visual input. The actions are one-hot-encoded and embedded in a vector which is multiplied channel-wise with the output of the convolutional layers. 
%Fully connected layers then process it and deconvolved. 
The network outputs the next frame of the game and the value of the reward.% Predicted rewards in \pong are $-1,0,1$ and are the same as in the original ALE environment (see Section \ref{sec:envs}). Predicted rewards  \breakout\ are $0$ and $1$: every positive reward is considered as $1$. Predicted rewards in the dense version of \freeway\ are $0$, $0.01$ and $1$. % We truncate rewards to $3$ possible values $in \pong:

% In most of our experiments we choose the input to be four frames as with our choice of environments they fully identify the state of the game. The network is the workhorse of our simulated environment $env'$. The environment contains a memory $M$ of four frames, which is initialized with frames retrieved from the real environment. Given an action, $a$ the tuple $(M,a)$ is processed by the network outputting a new frame and a reward $r$. The oldest frame of $M$ is discarded and the new one is included. 

%\todo{pm: The next section is too much of storytelling}
%\todo{you can shorten it and put the rest of details as a table}
% As shown in model-free experiments \cite{dqn,dqn2,ppo,acktr,rainbow,a3c}, using $4$ frames seems to be sufficient to train agents in a majority of Atari games and the same design decision we applied to neural network simulators. % the case of training of
% % Why $4$ frames? It is enough for reinforcement learning in many games.
% % Since in this work
% Another design decision concerned resizing and possible augmentation of the input frame marked as $X$ in Figure \ref{fig:kanapa}. We decided to feed the original $4$ RGB frames of the size $160\times 210$ pixels, meaning that a single input to the neural network is a tensor of the size $4 \times 160\times 210\times 3$ with a single cell of the tensor ranging from $0$ to $255$. In our design, the same is true about the output $X'$.
%\todo{Important: no pooling}

In our experiments, we varied details of the architecture above. In most cases, we use a stack of four convolutional layers with $64$ filters followed by three dense layers (the first two have $1024$ neurons). The dense layers are concatenated with $64$ dimensional vector with a learnable action embedding. Next, three deconvolutional layers of $64$ filters follow. An additional deconvolutional layer outputs an image of the original $105\times 80$ size. The number of filters is either $3$ or $3 \times 256$. In the first case, the output is a real-valued approximation of pixel's RGB value. In the second case, filters are followed by softmax producing a probability distribution on the color space. The reward is predicted by a softmax attached to the last fully connected layer. 
We used dropout equal to $0.2$ and layer normalization. 

\paragraph{Loss functions.}
The visual output of our networks is either one float per pixel/channel or the categorical 256-dimensional softmax. In both cases, we used the \textit{clipped loss} $\max(Loss, C)$ for a constant $C$. We found that clipping was crucial for improving the prediction power of the models (both measured with the correct reward predictions per sequence metric and successful training using Algorithm~\ref{dpll}). We conjecture that the clipping substantially decreases the magnitude of gradients stemming from fine-tuning of big areas of background consequently letting the optimization process concentrate on small but important areas (e.g. the ball in Pong). In our experiments, we set $C=10$ for $L_2$ loss on pixel values and to $C=0.03$ for softmax loss.
Note that this means that when the level of confidence about the correct pixel value exceeds $97\%$  (as $-\ln(0.97) \approx 0.03$) we get no gradients from that pixel any longer.

\paragraph{Scheduled sampling.}
The simulator $env'$ consumes its own predictions from previous steps. Thus, due to compounding errors, the model may drift out of the area of its applicability. Following \cite{BengioVJS15}, we mitigate this problem by randomly replacing in training some frames of the input $X$ by the prediction from the previous step. Typically, we linearly increase the mixing probability during training arriving at $100\%$.

\subsection{Stochastic Models}
%In stochastic environments, explicitly modeling the stochasticity of the environment is crucial for a quality world model. Although Atari is known as a deterministic environment, it can act stochastically in practical settings. The main source of such stochasticities is the limited number of input frames as well the sprite occlusion/flickering in the observed frames. 
A stochastic model can be used to deal with limited horizon of past observed frames as well as sprites occlusion and flickering which results to higher quality predictions. 


Inspired by~\citet{sv2p}, we used a variational autoencoder ~\citep{kingma2013auto} to model the stochasticity of the environment. In this model, an additional network receives the input frames as well as the future target frame as input and approximates the distribution of the posterior. At each timestep, a latent value $z_t$ is sampled from this distribution and will be passed as input to the original predictive model. At test time, the latent values are sampled from an assumed prior 
$\mathcal{N}(\mathbf{0}, \mathbf{I})$. 
To match the assumed prior and the approximate, we use the Kullback–Leibler divergence term as an additional loss term~\citep{sv2p}.


Nonetheless, we noticed two major issues with this model. First, the weight of KL divergence loss term is game dependent and has to be optimised as a hyper-parameter which is not practical if one wants to deal with a broad portfolio of Atari games. Second, this weight is usually a very small number in the range of $[e^{-5}, e^{-3}]$ which means that the approximated posterior can diverge significantly from the assumed prior. This can result in previously unseen latent values at inference time that lead to poor predictions. We address these issues by utilizing a discrete latent variable similar to~\citet{auto_discrete}. 

As visualized in Figure~\ref{fig:full_discrete}, the proposed stochastic model with discrete latent variables discretizes the latent values into bits (zeros and ones) while training an auxiliary LSTM-based~\cite{hochreiter1997long} recurrent network to predict these bits autoregressively. At inference time, the latent bits will be generated by this auxiliary network in contrast to sampling from a prior. To make the predictive model more robust to unseen latent bits, we add uniform noise to approximated latent values before discretization and apply dropout~\cite{srivastava2014dropout} on bits after discretization.
% Already in caption: Please note that similar to~\citet{neural_discrete},
% the backpropagation bypasses the discretization operation. 
% MB: move to appendix
% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{figures/model_basic_stoch.pdf}
% \caption{Architecture of stochastic model. The generative network is the same as Figure~\ref{fig:model_det} with an additional convolutional inference network to approximates the posterior given the next frame. The latent values will be sampled from approximated posterior and an assumed prior of $\mathcal{N}(\mathbf{0}, \mathbf{I})$ at training and inference time respectively.}
% \label{fig:model_stoch}
% \end{figure*}




==> learning_algorithm_old.tex <==
\section{Model based learning algorithm}
\label{subsec:model}

Reinforcement learning is formalized by Markov decision processes (MDP). An MDP is defined as a tuple $(\mathcal{S}, \Aa, P, r, \gamma)$, where $\mathcal{S}$ is a state space, $\Aa$ is a set of actions available to an agent, $P$ is the transition kernel, $r$ is reward function and $\gamma\in (0,1)$ is the discount factor. 

In this work we refer to MDPs as environments and assume that environments fulfill the following assumptions:
(1) Our environments do not have direct access to the state (i.e., the RAM of Atari 2600 emulator). Instead we use visual observations, typically $210\times 160$ RGB images. A single image does not determine the state. To circumvent this we stack the four previous frames. After this augmentations we will assume that the observation can be identified with the state.
%%SL.1.15: can probably remove that last sentence -- since the model is recurrent anyway, I'm not sure we even need this assumption
(2) Our environments are deterministic, namely the transition kernel $P$ can be identified with a function $env:\mathcal{S}\times \Aa\mapsto \mathcal{S}$, i.e. given a state and action the environment produces the next state.
%%SL.1.15: do we actually need this assumption?
(3) The action space $\Aa$ and the space of rewards are finite. 

A reinforcement learning agent interacts with the MDP issuing actions according to a policy. Formally, policy $\pi$ is a mapping from states to probability distributions over $\mathcal{A}$. The quality of a policy is measured by the value function $\mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s_0=s \right)$, which for a starting state $s$ estimates the total discounted reward gathered by the agent. In Atari 2600 games our goal is to find a policy which maximizes the value function when the starting state is the beginning of the game.

Crucially, apart from a Atari 2600 emulator environment $env$ we will use \textit{a neural network simulated environment} $env'$. The environment $env'$ shares the action and reward spaces with $env$ and produces visual observations in the same format. The  environment $env'$ will be trained to mimic $env$.  The principal aim of our work is to check
%%SL.1.15: well, maybe not just to check -- perhaps we can say The principal aim of our work is to train a policy...
if one can 
train a policy $\pi$ using a simulated environment $env'$ so that $\pi$ achieves a desired performance in the original environment $env$. During the training we aim to use as little interactions with $env$ as possible. 


The initial data to train $env'$ comes from random rollouts of $env$. As this is unlikely to capture all aspects of the environment, thus we use the following data-aggregation iterative algorithm inspired by Section 4 in  \cite{trpo_ensemble} and Section 5 in \cite{world_models}.
%%SL.1.15: To be fair, this basic scheme has been in use for decades and is basically ubiquitous for model-based RL. Feels odd to credit it to two papers from the last couple of years.

%\begin{figure*}[H]
\begin{algorithm}[H]
\caption{Pseudocode for model-based RL}\label{dpll}
\begin{algorithmic}
\STATE Initialize policy $\boldsymbol\pi$
\STATE Initialize model parameters $env'$
\STATE Initialize empty set $\mathbf{D}$
\WHILE{not done} 
\STATE \underline{$\triangleright$ collect observations from real env.}
\WHILE{not enough observations}
\STATE $(\mathbf{state},\mathbf{reward}) \gets env(\boldsymbol\pi(\mathbf{state}))$
\STATE $\mathbf{D} \gets \mathbf{D} \cup (\mathbf{state},\mathbf{reward})$
\ENDWHILE
\STATE \underline{$\triangleright$ update model using collected data.}
\STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env`, \mathbf{D})$
\STATE \underline{$\triangleright$ update policy using world model.}
\STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, \boldsymbol\theta)$
\ENDWHILE
\end{algorithmic}
\label{basic_loop}
\label{alg:basic_loop}
\end{algorithm}
% \end{figure*}

==> learning_algorithm_old_v2.tex <==
\section{Model based learning algorithm}
\label{subsec:model}

Reinforcement learning is formalized by Markov decision processes (MDP). An MDP is defined as a tuple $(\mathcal{S}, \Aa, P, r, \gamma)$, where $\mathcal{S}$ is a state space, $\Aa$ is a set of actions available to an agent, $P$ is the transition kernel, $r$ is reward function and $\gamma\in (0,1)$ is the discount factor. 

In this work we refer to MDPs as environments and assume % that environments fulfill the following assumptions:
that environments do not have direct access to the state (i.e., the RAM of Atari 2600 emulator). Instead we use visual observations, typically $210\times 160$ RGB images. A single image does not determine the state. To circumvent this we stack the four previous frames.
% \todo[inline]{BO.1.21: Maybe it would be worth to add a footnote explaining that four previous frames is not always sufficient to capture the state? Or have a section on this in latter chapter and here just refer to it?}
%5(2) Our environments are deterministic, namely the transition kernel $P$ can be identified with a function $env:\mathcal{S}\times \Aa\mapsto \mathcal{S}$, i.e. given a state and action the environment produces the next state.
% \todo[inline]{LK.1.22: I think we don't need this assumption as we're using stochastic models now, right? Can we remove it?}
%%SL.1.15: do we actually need this assumption?
(3) The action space $\Aa$ and the space of rewards are finite. 

A reinforcement learning agent interacts with the MDP issuing actions according to a policy. Formally, policy $\pi$ is a mapping from states to probability distributions over $\mathcal{A}$. The quality of a policy is measured by the value function $\mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s_0=s \right)$, which for a starting state $s$ estimates the total discounted reward gathered by the agent. In Atari 2600 games our goal is to find a policy which maximizes the value function when the starting state is the beginning of the game.

Crucially, apart from a Atari 2600 emulator environment $env$ we will use \textit{a neural network simulated environment} $env'$. The environment $env'$ shares the action and reward spaces with $env$ and produces visual observations in the same format. The  environment $env'$ will be trained to mimic $env$.  The principal aim of our work is to
train a policy $\pi$ using a simulated environment $env'$ so that $\pi$ achieves a desired performance in the original environment $env$. During the training we aim to use as few interactions with $env$ as possible. 


The initial data to train $env'$ comes from random rollouts of $env$. As this is unlikely to capture all aspects of the environment, thus we use the data-aggregation iterative algorithm presented in Algorithm~\ref{alg:basic_loop}.
\begin{figure}
\removelatexerror
\begin{algorithm}[H]
\caption{Pseudocode for model-based RL}\label{dpll}
\begin{algorithmic}
\STATE Initialize policy $\boldsymbol\pi$
\STATE Initialize model parameters $env'$
\STATE Initialize empty set $\mathbf{D}$
\WHILE{not done} 
\STATE \underline{$\triangleright$ collect observations from real env.}
\WHILE{not enough observations}
\STATE $(\mathbf{state},\mathbf{reward}) \gets env(\boldsymbol\pi(\mathbf{state}))$
\STATE $\mathbf{D} \gets \mathbf{D} \cup (\mathbf{state},\mathbf{reward})$
\ENDWHILE
\STATE \underline{$\triangleright$ update model using collected data.}
\STATE $\boldsymbol\theta \gets \text{TRAIN\_SUPERVISED}(env`, \mathbf{D})$
\STATE \underline{$\triangleright$ update policy using world model.}
\STATE $\boldsymbol\pi \gets \text{TRAIN\_RL}(\boldsymbol\pi, \boldsymbol\theta)$
\ENDWHILE
\end{algorithmic}
\label{basic_loop}
\label{alg:basic_loop}
\end{algorithm}
\end{figure}

==> related_work_old.tex <==
\section{Related work}
\label{sec:related_work}

% \paragraph{Model-free algorithms and Atari games.} 
In \cite{dqn} the authors presented the DQN algorithm which learns to play a large number of Atari games. The algorithm was extended in \cite{ppo,acktr,dqn2,rainbow,a3c} towards higher performance and better parallelization. % and in \cite{acktr} towards sample efficiency. % \todo[inline]{Add more "sample efficient" methods?} % emphasizes sample efficiency and in a number of games achieves the state-of-the-art performance utilizing only 2 million frames. Other above mentioned algorithms tend to utilize at least an order of magnitude more frames to achieve the top performance. 
%%SL.12.27:  Maybe it would be good to put this paragraph first in this section, as a way to motivate and set up the problem? That would then flow nicely into model-based RL, where the end of this paragraph can state clearly the model-free RL challenges.
In this work we are addressing a question what kind of performance in Atari games can be achieved within the budget of 100K frames. None of the above methods was tested against such a strict sample efficiency requirement, hence in this work we include a thorough evaluation of the PPO \cite{ppo} and Rainbow \cite{rainbow} algorithms optimized for performance on 100K and 1M frames, see Table \ref{table:rainbow}.

% \paragraph{Model-based methods.}  
% The budget of 100K frames is spent on learning of the model of environment.  
In \cite{recurrent,video_prediction} it is shown that learning of Atari 2600 environments is possible using appropriately chosen deep learning architectures. Impressively, in some cases the predictions maintain high $L_2$ accuracy over timespans of hundreds steps. % Learning of rewards is not reported.
%%SL.12.27: I understand why that last sentence is important, but it feels somehow passive aggressive. Maybe we can just remove it and make everyone happier?
%%CF.12.27: What we could do is later phrase that, unlike prior work, we focus on using video prediction in the context of learning the play the game well.
As learned simulators of Atari environments are core ingredients of our approach, in many aspects our work is motivated by \cite{recurrent,video_prediction}, however we focus on using video prediction in the context of learning how to play the game well and positively verify that learned simulators can be used to train a policy useful in original environments. In other terms we are making a step from a pure video-prediction task in \cite{recurrent,video_prediction} to a model-based learning for Atari games. 
Perhaps surprisingly, there is virtually no work on model-based learning in video games. A notable exception is 
%an interesting new work 
\cite{world_models}. The authors compose variational autoencoders with recurrent neural networks into an architecture being able to model evolution of non-deterministic games. This architecture is successfully evaluated in the VizDoom environment on a task which requires avoiding random fireballs. They propose a training procedure, which is essentially the same as Algorithm \ref{alg:basic_loop}. In the VizDoom experiment they need only one loop as the environment has rather dense rewards and is simple enough to be discovered by random exploration. % Interestingly, they increase the randomness of the simulator to prevent training from exploiting loopholes of the neural network model.

For a survey of model-based methods for robotics see \cite[Chapter 3]{deisenroth}. In this domain recent works  \cite{finn2016, ebert, hafner, piergiovanni, paxton, rybkin-pertsch}  are focused on learning models from raw pixels and our approach to learning of models in Atari games is closely motivated by this line of research, see Section \ref{sec:architectures} for detailed description of our models used for video and reward predictions.  Another source of motivation is a stochastic video prediction model \cite{sv2p} and discrete autoencoders described in \cite{neural_discrete, auto_discrete}.   % In \cite{trpo_ensemble} the model-based approach is applied in the context of the MuJoCo physics simulator \cite{mujoco}. 

In a recent work \cite{trpo_ensemble} a training loop similar to one described in  Algorithm \ref{basic_loop} along with a policy gradient algorithm \cite{trpo} was applied to a number of robotic tasks in the MuJoCo physics simulator \cite{mujoco}. Learning in  \cite{trpo_ensemble} is based on the state of the robot and does not involve visual inputs. 

% \paragraph{Augmenting model-free reinforcement learning using a model.} In \cite{imagination_metacontrol,imagination_model_based_planning} a model of the environment called {\em imagination} is used to augment performance of a model-free reinforcement learning algorithm. This proved to be particularly useful in games like Sokoban, where certain moves are irreversible. 
% HM.1.9:  removing imagination to save space, also it does not involve Atari

%There are number of differences though. We argue that the $L_2$ accuracy is not necessarily a good proxy measure for assessing applicability in reinforcement learning. Instead we argue for using \textit{correct rewards per sequence} metric (see Section \ref{sec:architectures}). In fact we found that training models with poor $L_2$ accuracy might be beneficial for \textit{correct rewards per sequence} metric as explained in Section \ref{sec:architectures}.
%%SL.12.27: I think this statement perhaps places somewhat undue emphasis on the metric. I can see the importance, but coming this early in the paper, readers might misunderstand it as suggesting that this is the key component that makes the method work at all...
% Finally, we positively verify that our simulations can be used to train a policy useful in original environments. 
% \paragraph{Learning models from pixels.} In \cite{pixel1, pixel2, pixel3, raw_visual}
%%SL.12.27: the first two are not concerned with robotics, the third one is robotics but doesn't learn models on pixels, and the fourth one is on pixels but doesn't learn models :) Chelsea can probably suggest the right related work to put here, but maybe what I might suggest is to first have a block of citations about model-based RL in general (whether from pixels or not), and cite the Deisenroth survey paper there, and then have a block of citations on learning models from pixels and cite papers that do that all together (Chelsea can probably provide this list)
%%CF.12.27: The relevant citations for model-based RL with raw pixel input is:
% -- Learn autoencoder on pixels and learn model in latent space: embed to control (Watter et al), deep spatial autoencoders (Finn et al), Danijar Hafner's latest paper (https://arxiv.org/abs/1811.04551)
% -- Learn model in pixel space and use it for planning and control: deep visual foresight (Finn et al.), self-supervised visual planning (Ebert et al), 
% -- this paper: https://arxiv.org/abs/1806.09655
% -- this paper: https://arxiv.org/abs/1805.07813
% -- this paper: https://arxiv.org/abs/1804.00062 (trains video predictor on demonstrations, not on autonomously collected data, so not really doing model-based RL, but still using video prediction)
% the model-based approach is applied to robotics. Models are taking images as inputs and  policies are trained to perform tasks such as moving a robotic arm or grasping of an object. In this work we focus on Atari games. This  standard reinforcement learning benchmark allows for an easy comparison of obtained results with the state-of-the-art achieved by model-free reinforcement learning algorithms.

% \paragraph{Learning of models in other games.} 
%%SL.12.27: I feel like we are better off having a more general discussion of related work on model-based reinforcement learning from pixels and adding this paper as one of the citations -- there are plenty of papers that do essentially the same thing, so it feels weird to single it out for an entire paragraph just because it's from Google (or for any other reason). For example, the e2c paper also uses VAEs.
%%CF.12.27: I agree that it doesn't make sense to separate this from the papers above. It belongs in the same category as embed-to-control/E2C, which I mentioned above.
%%HM.6.01: I agree with the criticism to some extend and will attempt to re-write it, but the main reason why it occupies so much space is that we are doing video games and the cited paper is the only one which also does video games. Besides, when we have started to talk with LK about the current project in Nov 2017, LK was aware of progress and of limitations of David's project and our work was intended to address some of these limitations. 

% \paragraph{Learning models from the state of a physics simulator.} In \cite{trpo_ensemble, mpc_model_based} the model-based approach is applied in the context of the MuJoCo physics simulator \cite{mujoco}. The simulator exposes the state of the environment which is in practice a vector of floats of length up to $50$. Authors of \cite{trpo_ensemble, mpc_model_based} use a data collection method similar to the one described in Algorithm \ref{basic_loop}.
%%SL.12.27: there are something like three decades of research on model-based RL algorithms... maybe a better scoping for related work would be to just cite the deisenroth survey and a couple recent papers (first) and then mostly focus on the pixel-based methods?

%(the latter has a good bibliography review for robotics)
%Missing bibliography \todo[inline]{Include the work on MuJoCo into the bibliography - they are in a separated model-based doc https://docs.google.com/document/d/1rjLmIoAGINii97cUCkSPcse61veQqd27wzEoOmL-Etc/edit?usp=sharing }
%%HM 6.01 trpo_ensemble has a unique (?) feature that iterated TRPO is used to learn policy. I consider this as an approval/precedence which justifies usage of PPO in our loop.   

% \paragraph{Augmenting model-free reinforcement learning using a model.} In \cite{imagination_metacontrol,imagination_model_based_planning} a model of the environment called {\em imagination} is used to augment performance of a model-free reinforcement learning algorithm. This proved to be particularly useful in games like Sokoban, where certain moves are irreversible. 
%%SL.12.27: For this kind of thing, it would be a good idea at the end of each section to discuss how this work relates to the current one. But also this paragraph can probably be cut (you'll be out of space)
%%HM 6.01 The reason these paper are cited here is that they are about video games and at the same time they use some ideas from model-based RL.

% \paragraph{Neural architectures suitable for modeling of video games. } In this work we apply two advanced recurrent models: the Stochastic Variational Video Prediction (SV2P, \cite{sv2p}) and a video discrete autoencoder inspired by \cite{neural_discrete, auto_discrete}. 
% PM.01.08 possibly add  \cite{Buesingatal2018}


%\paragraph{Use of autoencoders.} We want a nice compact representation and run our reinforcement learning algorithm on the representation. \todo[inline]{This appears in quite a few places including \cite{raw_visual,world_models,deep_spatial,embed_to_control} but also some of pixel series \cite{pixel1,pixel2,pixel3}}

%\paragraph{Encouraging exploration.} Certainly this idea appers in \cite{video_prediction}. See also \href{http://rll.berkeley.edu/deeprlcourse/f17docs/advanced_model_learning.pdf#29}{Notes from the Berkeley course, page 29.}




% \todo[inline]{Include discussion of 3 papers mentioned in notes.}

%\todo[inline]{It would be good to find a source which really measures sample efficiency.}

%\paragraph{Worth of including here.} Schmidhuber-Huber \cite{huber} Bellemare, PhD thesis \cite{marc_skip,marc_bayesian_learning}; these all appears in related work in \cite{video_prediction}.

==> related_work_old_v2.tex <==
\section{Related work}
\label{sec:related_work}

% HM.1.9. a version of old related work section is in the file related_work_old.tex.
% It includes all comments, but sadly I have mingled/misplaced them in the process of re-writing.
% I am maintaining the distinction "video games vs robotics", but if necessary I am ready to drop it

%%SL.1.15: Here is a rephrasing that maintains the spirit of the original but somewhat emphasizes the distinction: Atari games gained prominence as a popular benchmark for reinforcement learning algorithms with the introduction of the Arcade Learning Environment (ALE)~\cite{}. The combination of reinforcement learning and deep models then enabled RL algorithms to learn to play Atari games directly from images of the game screen, using the DQN algorithm~\cite{dqn}, policy gradients~\cite{}, and actor-critic algorithms~\cite{}. The most successful methods in this domain remain model-free algorithms~\cite{rainbow?}. However, although the sample complexity of these methods has improved substantially over the last few years, it remains far higher than the amount of experience required for human players to learn each game~\cite{}. In this work, we aim to learn Atari games with a budget of just 100K frames, corresponding to one hour of play time. Prior methods are generally not evaluated in this regime, and we therefore reoptimized two prior methods: PPO~\cite{ppo} and Rainbow~\cite{rainbow} for optimal performance on 100K and 1M frames for comparison.
In a number of Atari games, impressive results have been achieved by the DQN algorithm \cite{dqn}. The algorithm was extended in \cite{ppo,acktr,dqn2,rainbow,a3c} towards higher performance and better parallelization.
In this work we are addressing a question what kind of performance in Atari games can be achieved within the budget of 100K frames. None of the above methods was tested against such a strict sample efficiency requirement, hence in this work we include a thorough evaluation of the PPO \cite{ppo} and Rainbow \cite{rainbow} algorithms optimized for performance on 100K and 1M frames, see Table \ref{table:rainbow}.\todo[inline]{HM @ Blazej: let us not forget about the table}

%%SL.1.15: Maybe we transition by saying: While to our knowledge no prior work has successfully learned to play a variety of Atari games with model-based reinforcement learning methods directly, multiple prior works have studied the problem of modeling Atari games, both as static videos and with action-conditioned models...
In \cite{video_prediction, recurrent} it is shown that learning of Atari 2600 environments is possible using appropriately chosen deep learning architectures. Impressively, in some cases the predictions maintain high $L_2$ accuracy over timespans of hundreds of steps. 
As learned simulators of Atari environments are core ingredients of our approach, in many aspects our work is motivated by \cite{video_prediction, recurrent}, however we focus on using video prediction in the context of learning how to play the game well and positively verify that learned simulators can be used to train a policy useful in original environments. In other terms we are making a step from a pure video-prediction task in \cite{video_prediction, recurrent} to model-based learning for Atari games.
%%SL.1.15: can probably cut this last sentence
An important step in this direction was made in \cite{video_reward_prediction}, which extends \cite{video_prediction} by including reward prediction, but does not use the model to learn policies that play the games.
Perhaps surprisingly, there is virtually no work on model-based RL in video games.
%%SL.1.15: should we say "from images"?
A notable exceptions are 
\cite{vpn,world_models}. In \cite{vpn} a model of rewards is used to augment model-free learning with good results on a number of Atari games, but the RL algorithm is not intended to be sample efficient.
%%SL.1.15: maybe instead of "but the ..." say "However, this method does not actually aim to model or predict future frames, and achieves clear but relatively modest gains in efficiency."
In \cite{world_models} a variational autoencoder is composed with a recurrent neural network into an architecture  
which is successfully evaluated in the VizDoom environment and on a 2D racing game. 
The training procedure is similar to  Algorithm \ref{alg:basic_loop}, but only one step of the loop is needed as the environments are simple enough to be fully explored with random exploration.
%%SL.1.15: I don't suppose there is anything we can include in our experiments that we can honestly say is a *comparison* to this method?

%%SL.1.15: Maybe a transition could go like this: Outside of games, model-based reinforcement learning has been explored at length for applications such as robotics~\cite{}. Though most such prior methods did not employ image observations, several recent works have sought to incorporate images into simulated~\cite{} and real-world~\cite{} robotic control.
For a survey of model-based methods for robotics see Chapter 3 in \cite{deisenroth}.
Our models of Atari environments described in Section \ref{sec:architectures} are motivated by video models developed for robotics applications in \cite{embed_to_control, deep_spatial, finn2016, sv2p, ebert, hafner, piergiovanni, paxton, rybkin-pertsch}.  Another source of an inspiration are discrete autoencoders proposed in \cite{neural_discrete, auto_discrete}.
%%SL.1.15: For this last sentence, I feel like we should instead have a separate place where we discuss related work on modeling (i.e., related prediction models)

%%SL.1.15: I think this paragraph can be merged into the discussion of model-based RL in robotics in the paragraph above. But if we want a paragraph on model-based RL methods that combine model-free optimizers and models, we can say something like this: The structure of the model-based RL algorithm that we employ consists of alternating between learning a model, and then using this model to optimize a policy by using model-free reinforcement learning within the model. Variants of this basic structure has been proposed in a number of prior works, ranging from Dyna~\cite{sutton_dyna_paper} to more recent methods that incorporate deep networks for models and policies... [and can cite/discuss here the ensemble paper (i.e., the discussion below), as well as stochastic value gradients, model-based value expansion, and this paper: Kalweit, Gabriel and Boedecker, Joschka. Uncertainty driven imagination for continuous deep reinforcement learning]
In a recent work \cite{trpo_ensemble} a training loop similar to one described in  Algorithm \ref{basic_loop} along with a policy gradient algorithm \cite{trpo} were applied to a number of robotic tasks in the MuJoCo physics simulator \cite{mujoco}.  This successful application of a learned model and a policy gradient algorithm motivated our choice of PPO \cite{ppo} as the algorithm which improves policy in the learned environment, see also discussion in Section 3.3.2.1 of \cite{deisenroth}. % "To the best our knowledge  knowledge, there are currently not many approaches for model-based policy  search  based  on  sampling-based  gradients  using  the  methods from Section 2."

% Two student papers on MBRL for Atari (Pong, specifically)
% http://cs231n.stanford.edu/reports/2016/pdfs/116_Report.pdf
% https://dspace.fandm.edu/bitstream/handle/11016/24289/Foley_Thesis.pdf?sequence=1&isAllowed=y
%%CF: I don't think we need to worry about citing these.

==> rl_algorithm.tex <==
\section{Reinforcement learning algorithm}
\label{sec:rl}

\textbf{pm: under construction do not change}

Given a stochastic policy $\pi$, which for a given state assigns probability distribution over possible actions, we define the value function $V_\pi(s) := \mathbb{E}_{\pi}\left(\sum_{t=0}^{+\infty}\gamma^t r_{t+1}|s=s_0 \right)$. We define $\eta(\pi)$ to be the value function, when the initial state is sampled according to $\rho_0$. The goal of reinforcement learning is to find a policy which maximizes $\eta$.

In our experiments the reinforcement learning part of the loop in Figure \ref{figure_basic_loop} (Algorithm \ref{basic_loop}, line 6) is performed with the Proximal Policy Optimization algorithm (PPO, \cite{ppo}). PPO is a general purpose model-free reinforcement learning algorithm. This kind of algorithm can be considered as a black-box in this project. The black-box works for a prescribed number of epochs. In a single epoch it gathers new episodes and using experience from the episodes it improves the policy. % The procedure is motivated by the DAgger algorithm \cite{dagger} and presented below in Algorithm \ref{basic_loop}.

\paragraph{Training of a reinforcement learning agent}
% TODO: details about PPO, update figure below.
% latex source https://www.overleaf.com/16266511yhyscgmyhztg
% \begin{figure}[H]
% \centering
% \includegraphics[width=4in]{figures/network_ppo.png}
%  \end{figure}

==> tikzlibrarynode-families.code.tex <==
\let\tikz@lib@nf@textheight\relax
\let\tikz@lib@nf@textdepth\relax
\let\tikz@lib@nf@textwidth\relax
\tikzset{
  Minimum Width/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@width}{}{%
      \tikzset{/tikz/minimum width/.expand twice=+\csname\pgfpictureid @#1@width\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerxsep{\pgfkeysvalueof{/pgf/outer xsep}}\global\let\tikz@lib@nf@outerxsep\tikz@lib@nf@outerxsep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{east}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{west}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \advance\pgf@x-\tikz@lib@nf@outerxsep
            \pgfutil@ifundefined{\pgfpictureid @#1@width}{%
              \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@width\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@width\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{width}{width}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Height/.code={%
    \pgfutil@ifundefined{\pgfpictureid @#1@height}{}{%
      \tikzset{/tikz/minimum height/.expand twice=+\csname\pgfpictureid @#1@height\endcsname}%
    }%
    \tikz@addmode{\pgfmathsetlengthmacro\tikz@lib@nf@outerysep{\pgfkeysvalueof{/pgf/outer ysep}}\global\let\tikz@lib@nf@outerysep\tikz@lib@nf@outerysep}%
    \tikzset{
      prefix after command={%
        \pgfextra
          \pgfinterruptpath
            \pgfsettransform{\csname pgf@sh@nt@\tikzlastnode\endcsname}%
            \pgfpointanchor{\tikzlastnode}{north}%
            \pgf@xa=\pgf@x \pgf@ya=\pgf@y
            \pgfpointanchor{\tikzlastnode}{south}%
            \advance\pgf@xa-\pgf@x
            \advance\pgf@ya-\pgf@y
            \pgfmathveclen@{\pgf@sys@tonumber\pgf@xa}{\pgf@sys@tonumber\pgf@ya}%
            \pgf@x\pgfmathresult pt\relax
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \advance\pgf@x-\tikz@lib@nf@outerysep
            \pgfutil@ifundefined{\pgfpictureid @#1@height}{%
              \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
            }{%
              \expandafter\ifdim\csname\pgfpictureid @#1@height\endcsname<\pgf@x
                \expandafter\xdef\csname\pgfpictureid @#1@height\endcsname{\the\pgf@x}%
              \fi
            }%
            \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
            \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\expandafter\tikz@lib@nf@save\expandafter{\pgfpictureid}{#1}{height}{height}}
          \endpgfinterruptpath
        \endpgfextra
      }%
    }%
  },
  Minimum Size/.style={
    Minimum Height={#1},
    Minimum Width={#1}},
  Text Height/.code=\edef\tikz@lib@nf@textheight{#1},
  Text Depth/.code= \edef\tikz@lib@nf@textdepth{#1},
  Text Width/.code=%
    \edef\tikz@lib@nf@textwidth{#1}%
    \pgfutil@ifundefined{\pgfpictureid @#1@textwidth}{}{%
      \tikzset{text width/.expand twice=+\csname\pgfpictureid @#1@textwidth\endcsname}%
    }%
}

\def\tikz@lib@nf@text@#1#2#3{%
  \expandafter\ifx\csname tikz@lib@nf@#3\endcsname\relax\else
    \ifx#1\wd\def\tikz@temp{@}\else\let\tikz@temp\pgfutil@empty\fi
    \expandafter\ifx\csname tikz@lib@nf@#3\tikz@temp\endcsname\pgfutil@empty\else
      \pgfutil@ifundefined{\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp}{%
        \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
      }{%
        \ifdim\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname<#1#2
          \expandafter\xdef\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\tikz@temp\endcsname{\the#1#2}%
        \else
          \ifx#1\wd\else
            #1#2=\csname\pgfpictureid @\csname tikz@lib@nf@#3\endcsname @#3\endcsname\relax
          \fi
        \fi
      }%
      \edef\tikz@temp{\noexpand\tikz@lib@nf@save{\pgfpictureid}{\csname tikz@lib@nf@#3\endcsname}{#3}{#3\tikz@temp}}%
      \expandafter\expandafter\expandafter\gdef\expandafter\expandafter\expandafter
      \tikz@atend@picture\expandafter\expandafter\expandafter{\expandafter\tikz@atend@picture\tikz@temp}%
    \fi
  \fi
}
%%% Redefinition
\def\tikz@fig@continue{%
    \ifx\tikz@text@width\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@width}%
      \wd\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@height\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@height}%
      \ht\pgfnodeparttextbox=\pgf@x%
    \fi%
    \ifx\tikz@text@depth\pgfutil@empty%
    \else%
      \pgfmathsetlength{\pgf@x}{\tikz@text@depth}%
      \dp\pgfnodeparttextbox=\pgf@x%
    \fi%
    %
    %
    %
    \tikz@lib@nf@text@\ht\pgfnodeparttextbox{textheight}%
    \tikz@lib@nf@text@\dp\pgfnodeparttextbox{textdepth}%
    \tikz@lib@nf@text@\wd\pgfnodeparttextbox{textwidth}%
    %
    % Node transformation
    %
    \tikz@node@transformations
    %
    \setbox\tikz@figbox=\hbox{%
      \setbox\pgfutil@tempboxa=\copy\tikz@figbox%
      \unhbox\pgfutil@tempboxa%
      \hbox{{%
          \pgfinterruptpath%
            \pgfscope%
              \tikz@options%
              \setbox\tikz@figbox=\box\pgfutil@voidb@x%
              \pgfmultipartnode{\tikz@shape}{\tikz@anchor}{\tikz@fig@name}{%
                \pgfutil@tempdima=\pgflinewidth%
                {\begingroup\tikz@finish}%
                \global\pgflinewidth=\pgfutil@tempdima%
              }%
            \endpgfscope
          \endpgfinterruptpath%
      }}%
    }%
    %
    \tikz@alias%
    \tikz@node@finish%
}
\def\tikz@lib@nf@save#1#2#3#4{%
  \pgfutil@ifundefined{#1@#2@#3@done}{%
    \expandafter\let\csname#1@#2@#3@done\endcsname\pgfutil@empty%
    \immediate\write\pgfutil@auxout{\noexpand\expandafter\noexpand\gdef\noexpand\csname#1@#2@#3\endcsname{\csname#1@#2@#4\endcsname}}
  }{}%
}
\endinput


==> tikzlibrarypositioning-plus.code.tex <==
% This is the TikZ library positioning-plus
% Load with \usetikzlibrary{positioning-plus}
%
% This small library extends TikZ options like 'above', 'left' or 'below right'
% so that they can be used with an optional prefixed factor seperated by ':' (colon)
%
% The option 'left=.5:of somenode' will place
% a new node .5cm (default 'node distance' is '1cm and 1cm') left to (somenode).
% The option 'above right=.2 and .7:of someothernode' will place
% a new node .2cm above and .7cm right of (someothernode).
%
% Additional the options 'xshift*' and 'yshift*' add an additional shift
% as a factor of 'node distance'
% Inspired by http://tex.stackexchange.com/a/117610/16595

\usetikzlibrary{positioning}
\usetikzlibrary{fit}

\pgfdeclaregenericanchor{corner south east}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north east}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{east}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner south west}{%
  \pgf@sh@reanchor{#1}{south}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}
\pgfdeclaregenericanchor{corner north west}{%
  \pgf@sh@reanchor{#1}{north}%
  \pgf@ya\pgf@y
  \pgf@process{\pgf@sh@reanchor{#1}{west}}%
  \pgf@y\pgf@ya
}

\tikzset{corner above left/.code=\tikz@lib@place@handle@{#1}{corner south east}{-1}{1}{corner north west}{0.707106781}}
\tikzset{corner above right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{1}{corner north east}{0.707106781}}
\tikzset{corner below left/.code=\tikz@lib@place@handle@{#1}{corner north east}{-1}{-1}{corner south west}{0.707106781}}
\tikzset{corner below right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{-1}{corner south east}{0.707106781}}

\tikzset{corner north left/.code =\tikz@lib@place@handle@{#1}{corner north east}{-1}{0}{corner north west}{1}}
\tikzset{corner north right/.code=\tikz@lib@place@handle@{#1}{corner north west}{1}{0}{corner north east}{1}}
\tikzset{corner south left/.code =\tikz@lib@place@handle@{#1}{corner south east}{-1}{0}{corner south west}{1}}
\tikzset{corner south right/.code=\tikz@lib@place@handle@{#1}{corner south west}{1}{0}{corner south east}{1}}

\tikzset{corner west above/.code =\tikz@lib@place@handle@{#1}{corner south west}{0}{1}{corner north west}{1}}
\tikzset{corner west below/.code=\tikz@lib@place@handle@{#1}{corner north west}{0}{-1}{corner south west}{1}}
\tikzset{corner east above/.code =\tikz@lib@place@handle@{#1}{corner south east}{0}{1}{corner north east}{1}}
\tikzset{corner east below/.code=\tikz@lib@place@handle@{#1}{corner north east}{0}{-1}{corner south east}{1}}

\tikzset{north left/.code =\tikz@lib@place@handle@{#1}{north east}{-1}{0}{north west}{1}}
\tikzset{north right/.code=\tikz@lib@place@handle@{#1}{north west}{1}{0}{north east}{1}}
\tikzset{south left/.code =\tikz@lib@place@handle@{#1}{south east}{-1}{0}{south west}{1}}
\tikzset{south right/.code=\tikz@lib@place@handle@{#1}{south west}{1}{0}{south east}{1}}

\tikzset{west above/.code =\tikz@lib@place@handle@{#1}{south west}{0}{1}{north west}{1}}
\tikzset{west below/.code=\tikz@lib@place@handle@{#1}{north west}{0}{-1}{south west}{1}}
\tikzset{east above/.code =\tikz@lib@place@handle@{#1}{south east}{0}{1}{north east}{1}}
\tikzset{east below/.code=\tikz@lib@place@handle@{#1}{north east}{0}{-1}{south east}{1}}

\newif\ifqrr@tikz@lib@place@postransform
\tikzset{node distance transformation/.is if=qrr@tikz@lib@place@postransform}
\def\tikz@lib@place@handle@@#1#2#3#4{%
  \pgfutil@in@{of }{#1}%
  \ifpgfutil@in@%
    \tikz@lib@place@of#1\tikz@stop{#4}%
  \else%
    \edef\tikz@lib@place@nums{#1}%
  \fi%
  \ifx\tikz@lib@place@nums\pgfutil@empty%
    % Ok, nothing to do, we have set the anchor and we are happy...
  \else%
    \expandafter\tikz@lib@place@parse@nums\expandafter{\tikz@lib@place@nums}%
    \pgf@x=#2\pgf@x%
    \pgf@y=#3\pgf@y%
    \ifqrr@tikz@lib@place@postransform
      \pgf@pos@transform{\pgf@x}{\pgf@y}% change from original
    \fi
    \edef\tikz@lib@pos@call{\noexpand\pgftransformshift{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}}%
  \fi%
}

\def\tikz@lib@place@handle@#1#2#3#4#5#6{%
  \pgfutil@in@{:}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@#1\tikz@stop
    \ifx\pgf@temp\pgfutil@empty
      \let\pgf@temp\tikz@node@distance
    \fi
    \pgfmathsetmacro\pgf@tempa{(\pgf@tempa)*#4}%
    \pgfmathsetmacro\pgf@tempb{(\pgf@tempb)*#3}%
    \edef\pgf@marshal{\noexpand\tikz@lib@place@handle@{\pgf@temp}{#2}{\pgf@tempb}{\pgf@tempa}{#5}{#6}}%
    \pgf@marshal
  \else
    \def\tikz@anchor{#2}%
    \let\tikz@do@auto@anchor=\relax%
    \edef\tikz@temp{#1}%
    \def\tikz@lib@place@single@factor{#6}%
    \expandafter\tikz@lib@place@handle@@\expandafter{\tikz@temp}{#3}{#4}{#5}%
  \fi
}
\def\tikz@lib@place@handle@qrr@#1:#2\tikz@stop{%
  \pgfutil@in@{and}{#1}%
  \ifpgfutil@in@
    \tikz@lib@place@handle@qrr@@#1\tikz@stop
  \else
    \tikz@lib@place@handle@qrr@@#1and#1\tikz@stop
  \fi
  \def\pgf@temp{#2}%
}
\def\tikz@lib@place@handle@qrr@@#1and#2\tikz@stop{%
  \def\pgf@tempa{#1}%
  \def\pgf@tempb{#2}%
}
\def\qrr@xyshift@starred#1#2#3{
  \edef\tikz@marshal{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
  \tikz@marshal
  \ifpgfutil@in@
    \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
  \else
    \let#3\tikz@node@distance
  \fi
  \pgfmathparse{(#1)*#3}%
  \ifpgfmathunitsdeclared
    \if#2x%
      \pgftransformshift{\pgfqpoint{\pgfmathresult pt}{0pt}}%
    \else
      \pgftransformshift{\pgfqpoint{0pt}{\pgfmathresult pt}}%
    \fi
  \else
    \ifx#2x
      \pgf@process{\pgfqpointxy{\pgfmathresult}{0}}%
    \else
      \pgf@process{\pgfqpointxy{0}{\pgfmathresult}}%
    \fi
    \pgftransformshift{\pgfqpoint{\pgf@x}{\pgf@y}}%
  \fi}
\tikzset{
  xshift*/.code=\qrr@xyshift@starred{#1}x\pgf@tempb,
  yshift*/.code=\qrr@xyshift@starred{#1}y\pgf@tempa,
}

\def\pgfutil@firstofmany#1#2\pgf@stop{#1}
\def\pgfutil@secondofmany#1#2\pgf@stop{#2}
\def\tikz@lib@place@of@#1#2#3{%
  \def\pgf@tempa{fit bounding box}%
  \edef\pgf@temp{\expandafter\pgfutil@firstofmany#2\pgf@stop}
  \if\pgf@temp(%
    \tikz@lib@place@fit@scan{#2}{0}%
  \else\if\pgf@temp|
      \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
    \else\ifx\pgf@temp\tikz@activebar
        \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{1}%
      \else\if\pgf@temp-
          \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{2}%
        \else\if\pgf@temp+
            \expandafter\tikz@lib@place@fit@scan\expandafter{\pgfutil@secondofmany#2\pgf@stop}{3}%
          \else
            \def\pgf@tempa{#2}%
          \fi
        \fi
      \fi
    \fi
  \fi
  \expandafter\tikz@scan@one@point\expandafter\tikz@lib@place@remember\expandafter(\pgf@tempa)%
  \iftikz@shapeborder%
    % Ok, this is relative to a border.
    \iftikz@lib@ignore@size%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{center}}%
      \def\tikz@anchor{center}%
    \else%
      \edef\tikz@node@at{\noexpand\pgfpointanchor{\tikz@shapeborder@name}{#3}}%
    \fi%
  \fi%
  \edef\tikz@lib@place@nums{#1}%
}
\def\tikz@lib@place@fit@scan#1#2{
  \pgf@xb=-16000pt\relax%
  \pgf@xa=16000pt\relax%
  \pgf@yb=-16000pt\relax%
  \pgf@ya=16000pt\relax%
  \if\pgfutil@firstofmany#1\pgf@stop(%
    \tikz@lib@fit@scan#1\pgf@stop%
  \else
    \tikz@lib@fit@scan(#1)\pgf@stop
  \fi
  \ifdim\pgf@xa>\pgf@xa
    % shouldn't happen
  \else
     \expandafter\def\csname pgf@sh@ns@fit bounding box\endcsname{rectangle}%
     \expandafter\edef\csname pgf@sh@np@fit bounding box\endcsname{%
       \def\noexpand\southwest{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}%
       \def\noexpand\northeast{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}%
     }%
     \expandafter\def\csname pgf@sh@nt@fit bounding box\endcsname{{1}{0}{0}{1}{0pt}{0pt}}%
     \expandafter\def\csname pgf@sh@pi@fit bounding box\endcsname{\pgfpictureid}%
     \ifcase#2\relax
     \or % 1 = vertical
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})}}}%
       \pgf@marshal
     \or % 2 = horizontal
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \or % 3 = both directions
       \pgf@y=\pgf@yb%
       \advance\pgf@y by-\pgf@ya%
       \pgf@x=\pgf@xb%
       \advance\pgf@x by-\pgf@xa%
       \edef\pgf@marshal{\noexpand\tikzset{minimum height={\the\pgf@y-2*(\noexpand\pgfkeysvalueof{/pgf/outer ysep})},minimum width={\the\pgf@x-2*(\noexpand\pgfkeysvalueof{/pgf/outer xsep})}}}%
       \pgf@marshal
     \fi
  \fi
}
\tikzset{
  fit bounding box/.code={\tikz@lib@place@fit@scan{#1}{0}},
  span vertical/.code={\tikz@lib@place@fit@scan{#1}{1}},
  span horizontal/.code={\tikz@lib@place@fit@scan{#1}{2}},
  span/.code={\tikz@lib@place@fit@scan{#1}{3}}}

\pgfmathdeclarefunction{x_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempb}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
\pgfmathdeclarefunction{y_node_dist}{0}{%
  \begingroup
    \edef\pgfmath@temp{\noexpand\pgfutil@in@{and}{\tikz@node@distance}}%
    \pgfmath@temp\ifpgfutil@in@
      \expandafter\tikz@lib@place@handle@qrr@@\tikz@node@distance\tikz@stop
    \else
      \edef\pgfmath@temp{\tikz@node@distance and\tikz@node@distance}%
      \expandafter\tikz@lib@place@handle@qrr@@\pgfmath@temp\tikz@stop
    \fi
    \pgfmathparse{\pgf@tempa}%
    \pgfmath@smuggleone\pgfmathresult
  \endgroup
}
%\tikzdeclarecoordinatesystem{node distance}{%
%  \tikz@cs@nd#1\tikz@stop}
%\def\tikz@cs@nd#1,#2\tikz@stop{%
%  \def\qrr@xyshift@starred@action##1{\pgftransformshift{##1}}%
%  \qrr@xyshift@starred{#1}x\pgf@tempb
%  \qrr@xyshift@starred{#2}y\pgf@tempa}
\endinput

